On Distribution Shift in Learning-based Bug Detectors

Deep learning has recently achieved initial success in program analysis tasks such as bug detection. Lacking real bugs, most existing works construct training and test data by injecting synthetic bugs into correct programs. Despite achieving high test accuracy (e.g., 90%), the resulting bug detectors are found to be surprisingly unusable in practice, i.e., <10% precision when used to scan real software repositories. In this work, we argue that this massive performance difference is caused by a distribution shift, i.e., a fundamental mismatch between the real bug distribution and the synthetic bug distribution used to train and evaluate the detectors. To address this key challenge, we propose to train a bug detector in two phases, first on a synthetic bug distribution to adapt the model to the bug detection domain, and then on a real bug distribution to drive the model towards the real distribution. During these two phases, we leverage a multi-task hierarchy, focal loss, and contrastive learning to further boost performance. We evaluate our approach extensively on three widely studied bug types, for which we construct new datasets carefully designed to capture the real bug distribution. The results demonstrate that our approach is practically effective and successfully mitigates the distribution shift: our learned detectors are highly performant on both our test set and the latest version of open source repositories. Our code, datasets, and models are publicly available at https://github.com/eth-sri/learning-real-bug-detector.

==> figures/real/argswap.tex <==
% cls ap
\addplot [draw=Peach, line width=0.7pt, densely dotted] coordinates {
  (0, 8.314032705)
  (1, 7.196785909)
  (2, 7.252536638)
  (4, 7.262829293)
  (8, 7.236793187)
  (16, 7.650756505)
  (32, 7.625114857)
  (64, 8.377211088)
  (100, 8.49)
};

% cls prec
\addplot [draw=Peach, line width=0.7pt] coordinates {
  (0, 1.31)
  (1, 28.360000000000003)
  (2, 25.64)
  (4, 42.42)
  (8, 58.330000000000005)
  (16, 28.57)
  (32, 50.0)
  (64, 47.06)
  (100, 73.68)
};

% cls recall
\addplot [draw=Peach, line width=0.7pt, dashed] coordinates {
  (0, 39.839999999999996)
  (1, 7.720000000000001)
  (2, 8.129999999999999)
  (4, 5.6899999999999995)
  (8, 5.6899999999999995)
  (16, 6.5)
  (32, 6.1)
  (64, 6.5)
  (100, 5.6899999999999995)
};

% cls-loc prec
\addplot [draw=Plum, line width=0.7pt] coordinates {
  (0, 1.0)
  (1, 26.87)
  (2, 24.36)
  (4, 42.42)
  (8, 58.330000000000005)
  (16, 28.57)
  (32, 50.0)
  (64, 47.06)
  (100, 73.68)  
};

% cls-loc recall
\addplot [draw=Plum, line width=0.7pt, dashed] coordinates {
  (0, 30.490000000000002)
  (1, 7.32)
  (2, 7.720000000000001)
  (4, 5.6899999999999995)
  (8, 5.6899999999999995)
  (16, 6.5)
  (32, 6.1)
  (64, 6.5)
  (100, 5.6899999999999995)
};

% cls-loc-rep prec
\addplot [draw=Cerulean, line width=0.7pt] coordinates {
  (0, 0.79)
  (1, 26.87)
  (2, 24.36)
  (4, 42.42)
  (8, 58.330000000000005)
  (16, 28.57)
  (32, 50.0)
  (64, 47.06)
  (100, 73.68)
};

% cls-loc-rep recall
\addplot [draw=Cerulean, line width=0.7pt, dashed] coordinates {
  (0, 23.98)
  (1, 7.32)
  (2, 7.720000000000001)
  (4, 5.6899999999999995)
  (8, 5.6899999999999995)
  (16, 6.5)
  (32, 6.1)
  (64, 6.5)
  (100, 5.6899999999999995)
};

==> figures/real/varmisuse.tex <==
% cls ap
\addplot [draw=Peach, line width=0.7pt, densely dotted] coordinates {
  (1, 5.969768152)
  (2, 5.687082124)
  (4, 7.312404672)
  (8, 10.14981819)
  (16, 9.629998123)
  (32, 13.95166061)
  (64, 17.52007739)
  (100, 20.96)
};

% cls prec
\addplot [draw=Peach, line width=0.7pt] coordinates {
  (0.8, 3.43)
  (2, 18.49)
  (4, 24.76)
  (8, 35.94)
  (16, 36.54)
  (32, 47.89)
  (64, 52.00)
  (100, 64.79)
};

% cls recall
\addplot [draw=Peach, line width=0.7pt, dashed] coordinates {
  (0.8, 35.42)
  (2, 6.55)
  (4, 7.74)
  (8, 6.85)
  (16, 5.65)
  (32, 10.12)
  (64, 11.61)
  (100, 13.69)
};

% cls-loc prec
\addplot [draw=Plum, line width=0.7pt] coordinates {
  (0.8, 2.45)
  (2, 16.81)
  (4, 22.86)
  (8, 34.38)
  (16, 32.69)
  (32, 45.07)
  (64, 49.33)
  (100, 61.97)
};

% cls-loc recall
\addplot [draw=Plum, line width=0.7pt, dashed] coordinates {
  (0.8, 25.30)
  (2, 5.95)
  (4, 7.14)
  (8, 6.55)
  (16, 5.06)
  (32, 9.52)
  (64, 11.01)
  (100, 13.10)
};

% cls-loc-rep prec
\addplot [draw=Cerulean, line width=0.7pt] coordinates {
  (0.8, 2.10)
  (2, 15.97)
  (4, 20.95)
  (8, 29.69)
  (16, 30.77)
  (32, 45.07)
  (64, 48.00)
  (100, 56.34)
};

% cls-loc-rep recall
\addplot [draw=Cerulean, line width=0.7pt, dashed] coordinates {
  (0.8, 21.73)
  (2, 5.65)
  (4, 6.55)
  (8, 5.65)
  (16, 4.76)
  (32, 9.52)
  (64, 10.71)
  (100, 11.90)
};

==> figures/real/wrongbinop.tex <==
% cls ap
\addplot [draw=Peach, line width=0.7pt, densely dotted] coordinates {
  (0, 9.669125659)
  (1, 11.44160093)
  (2, 12.49143545)
  (4, 20.92911059)
  (8, 23.68456504)
  (16, 29.85541751)
  (32, 33.8437303)
  (64, 33.05013896)
  (100, 39.85)
};

% cls prec
\addplot [draw=Peach, line width=0.7pt] coordinates {
  (0.8, 9.69)
  (2, 15.54)
  (4, 20.73)
  (8, 26.92)
  (16, 48.26)
  (32, 48.59)
  (64, 49.53)
  (100, 52.30)
};

% cls recall
\addplot [draw=Peach, line width=0.7pt, dashed] coordinates {
  (0.8, 49.08)
  (2, 18.74)
  (4, 3.46)
  (8, 4.28)
  (16, 31.16)
  (32, 38.49)
  (64, 43.38)
  (100, 43.99)
};

% cls-loc prec
\addplot [draw=Plum, line width=0.7pt] coordinates {
  (0.8, 8.93)
  (2, 14.70)
  (4, 20.73)
  (8, 26.92)
  (16, 47.63)
  (32, 47.81)
  (64, 48.37)
  (100, 51.09)
};

% cls-loc recall
\addplot [draw=Plum, line width=0.7pt, dashed] coordinates {
  (0.8, 45.21)
  (2, 17.72)
  (4, 3.46)
  (8, 4.28)
  (16, 30.75)
  (32, 37.88)
  (64, 42.36)
  (100, 42.97)
};

% cls-loc-rep prec
\addplot [draw=Cerulean, line width=0.7pt] coordinates {
  (0.8, 8.09)
  (2, 13.01)
  (4, 20.73)
  (8, 26.92)
  (16, 47.32)
  (32, 46.79)
  (64, 47.21)
  (100, 49.64)
};

% cls-loc-rep recall
\addplot [draw=Cerulean, line width=0.7pt, dashed] coordinates {
  (0.8, 40.94)
  (2, 15.68)
  (4, 3.46)
  (8, 4.28)
  (16, 30.55)
  (32, 37.07)
  (64, 41.34)
  (100, 41.75)
};

==> figures/rp/gnn/tex/gnn-pybuglab-argument-swap.tex <==

\nextgroupplot[
	title={(b) BugLab}
]
\addplot [draw=Plum, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.5555)
(96.3415,0.6555)
(88.2114,0.7555)
(70.3252,0.8556)
(61.3821,0.9556)
(57.7236,1.0557)
(51.6260,1.1557)
(46.7480,1.2557)
(39.0244,1.3557)
(27.6423,1.4558)
(25.2033,1.5558)
(22.3577,1.6561)
(21.1382,1.7562)
(20.3252,1.8567)
(17.0732,1.9571)
(14.2276,2.0576)
(13.4146,2.1583)
(13.0081,2.2583)
(12.6016,2.4012)
(12.1951,2.5021)
(11.7886,2.6079)
(11.3821,3.0769)
(10.9756,3.1802)
(10.5691,3.8748)
(9.7561,3.7094)
(9.3496,3.8143)
(8.9431,3.6728)
(8.5366,4.3933)
(8.1301,4.7733)
(7.7236,4.6683)
(7.3171,9.0000)
(6.9106,13.0769)
(6.5041,12.5000)
(6.0976,14.2857)
(5.6911,16.0920)
(5.2846,16.2500)
(4.8780,15.1899)
(4.4715,18.9655)
(4.0650,22.2222)
(3.6585,25.7143)
(3.2520,80.0000)
(2.8455,77.7778)
(2.4390,85.7143)
(2.0325,83.3333)
(1.6260,80.0000)
(1.2195,75.0000)
(0.8130,100.0000)
(0.0,100.0000)};\addplot [draw=Cerulean, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.5067)
(90.2439,0.6067)
(72.3577,0.7067)
(61.7886,0.8068)
(23.1707,0.9068)
(21.9512,1.0069)
(21.5447,1.1069)
(18.6992,1.2070)
(18.2927,1.3074)
(15.4472,1.4074)
(13.8211,1.5078)
(13.4146,1.7685)
(9.3496,1.6655)
(8.9431,1.7657)
(8.5366,1.8667)
(8.1301,2.1482)
(7.7236,2.2485)
(6.9106,2.1411)
(6.5041,2.4096)
(6.0976,2.5126)
(5.6911,2.8986)
(5.2846,3.5912)
(4.4715,3.2934)
(4.0650,3.4014)
(3.6585,4.9724)
(3.2520,5.3691)
(2.8455,4.9296)
(2.4390,5.0420)
(2.0325,4.3478)
(1.6260,17.3913)
(1.2195,13.6364)
(0.8130,18.1818)
(0.4065,14.2857)
(0.0000,0.0000)
(0.0,0.0000)};\addlegendentry{GNN (BugLab + Real) (AP = 5.14)}
\addlegendentry{GNN (Only BugLab) (AP = 1.52)}


==> figures/rp/gnn/tex/gnn-pybuglab-var-misuse.tex <==

\nextgroupplot[
	title={(d) \varmisuse{} (BugLab)}
]
\addplot [draw=Plum, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.7287)
(99.7024,0.8287)
(98.5119,0.9287)
(97.3214,1.0287)
(95.5357,1.1287)
(95.2381,1.2287)
(93.7500,1.3288)
(91.3690,1.4288)
(89.2857,1.5289)
(88.3929,1.6289)
(83.9286,1.7290)
(82.1429,1.8290)
(80.3571,1.9291)
(77.6786,2.0292)
(74.7024,2.1293)
(72.9167,2.2293)
(65.1786,2.3295)
(64.2857,2.4297)
(61.6071,2.5299)
(58.9286,2.6302)
(50.0000,2.7304)
(48.8095,2.8305)
(41.3690,2.9306)
(40.7738,3.0310)
(32.4405,3.1313)
(31.8452,3.2317)
(30.9524,3.3323)
(22.6190,3.4327)
(20.8333,3.5336)
(19.3452,3.4067)
(17.8571,3.2949)
(17.5595,3.3967)
(16.0714,3.4974)
(15.1786,3.5992)
(13.3929,3.7007)
(12.7976,3.8019)
(12.5000,3.9033)
(11.9048,3.7987)
(11.6071,4.0289)
(11.3095,4.1989)
(10.7143,4.0314)
(10.4167,4.1322)
(10.1190,4.2341)
(9.8214,4.3364)
(9.5238,4.4383)
(9.2262,4.5388)
(8.9286,4.6656)
(8.6310,4.7776)
(8.0357,4.6713)
(7.7381,4.5614)
(7.4405,4.4563)
(7.1429,4.5627)
(6.5476,4.4177)
(6.2500,4.6875)
(5.9524,5.6818)
(5.6548,5.4131)
(5.3571,5.5215)
(5.0595,5.6291)
(4.7619,5.3691)
(4.4643,5.7252)
(4.1667,7.7348)
(3.8690,7.9755)
(3.5714,7.6923)
(3.2738,8.0882)
(2.9762,8.1967)
(2.6786,8.6538)
(2.3810,12.6984)
(2.0833,11.8644)
(1.7857,11.1111)
(1.4881,12.8205)
(1.1905,16.0000)
(0.8929,33.3333)
(0.5952,40.0000)
(0.2976,100.0000)
(0.0,100.0000)};\addplot [draw=Cerulean, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.7011)
(96.1310,0.8011)
(89.8810,0.9011)
(74.4048,1.0011)
(64.2857,1.1011)
(40.7738,1.2012)
(30.6548,1.3013)
(22.6190,1.4014)
(19.0476,1.5016)
(14.5833,1.3944)
(14.2857,1.4949)
(13.9881,1.6019)
(8.3333,1.4690)
(8.0357,1.5734)
(7.4405,1.6745)
(7.1429,1.7751)
(6.2500,1.8767)
(5.6548,1.7336)
(5.3571,1.8349)
(5.0595,1.9362)
(4.7619,2.0382)
(4.4643,1.9355)
(3.8690,1.8156)
(3.5714,2.1127)
(3.2738,2.2587)
(2.9762,2.3641)
(2.6786,2.6786)
(2.3810,2.7875)
(2.0833,2.6316)
(1.7857,3.7267)
(1.4881,11.3636)
(1.1905,13.3333)
(0.8929,13.6364)
(0.5952,15.3846)
(0.2976,20.0000)
(0.0000,0.0000)
(0.0,0.0000)};\addlegendentry{GNN (BugLab + Real) (AP = 3.84)}
\addlegendentry{GNN (Only BugLab) (AP = 1.60)}


==> figures/rp/gnn/tex/gnn-pybuglab-wrong-binary-operator.tex <==

\nextgroupplot[
	title={(e) \wrongbinop{} (BugLab)}
]
\addplot [draw=Plum, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,1.4823)
(99.5927,1.5823)
(99.1853,1.6823)
(98.9817,1.7824)
(98.7780,1.8824)
(98.3707,1.9824)
(98.1670,2.0825)
(97.9633,2.1826)
(97.1487,2.2827)
(96.9450,2.3827)
(96.3340,2.4828)
(95.3157,2.5829)
(95.1120,2.7477)
(94.2974,2.8478)
(94.0937,2.9479)
(93.8900,3.0479)
(93.4827,3.1481)
(93.0754,3.2483)
(92.2607,3.3484)
(91.6497,3.4485)
(91.0387,3.5487)
(90.6314,3.6490)
(90.2240,3.7492)
(89.6130,3.8492)
(89.4094,3.9493)
(89.0020,4.0493)
(88.5947,4.1496)
(87.9837,4.2499)
(87.7800,4.3500)
(86.9654,4.4502)
(86.7617,4.5503)
(86.5580,4.6504)
(85.7434,4.7506)
(84.9287,4.8511)
(84.7251,4.9654)
(84.5214,5.0659)
(83.7067,5.1666)
(83.5031,5.2672)
(83.0957,5.3677)
(82.8921,5.4682)
(82.6884,5.5685)
(82.2811,5.6686)
(81.8737,5.7692)
(81.6701,5.8893)
(80.6517,5.9900)
(80.4481,6.0900)
(79.6334,6.1906)
(79.2261,6.2914)
(79.0224,6.3921)
(78.8187,6.5316)
(78.6151,6.6323)
(78.0041,6.7335)
(77.8004,6.9518)
(77.5967,7.0805)
(77.3931,7.1807)
(77.1894,7.3279)
(76.5784,7.4294)
(76.3747,7.5301)
(75.9674,7.6309)
(75.7637,7.7938)
(75.5601,7.8953)
(75.3564,7.9965)
(74.7454,8.0980)
(74.5418,8.1989)
(74.1344,8.2991)
(73.9308,8.4047)
(73.7271,8.5986)
(72.9124,8.6999)
(72.5051,8.8010)
(71.6904,8.9024)
(71.4868,9.0745)
(71.2831,9.2300)
(71.0794,9.3316)
(70.8758,9.4823)
(70.6721,9.5936)
(70.4684,9.6946)
(70.2648,9.7956)
(70.0611,9.8964)
(69.8574,9.9971)
(69.6538,10.0974)
(69.4501,10.2280)
(69.2464,10.3281)
(69.0428,10.4308)
(68.8391,10.5625)
(68.6354,10.6646)
(68.4318,11.0490)
(68.2281,11.4726)
(67.8208,11.5746)
(67.6171,12.0771)
(67.4134,12.1781)
(67.2098,12.3503)
(67.0061,12.5429)
(66.8024,12.6446)
(66.5988,12.7485)
(66.3951,12.8498)
(66.1914,13.0365)
(65.9878,13.1387)
(65.7841,13.3306)
(65.5804,13.4447)
(65.3768,13.5500)
(65.1731,13.6752)
(64.9695,13.9058)
(64.7658,14.0088)
(64.5621,14.1140)
(64.3585,14.2150)
(64.1548,14.6375)
(63.7475,14.7433)
(63.5438,15.0144)
(63.3401,15.1191)
(63.1365,15.6014)
(62.9328,16.0770)
(62.7291,16.1850)
(62.5255,16.7851)
(62.3218,16.8874)
(61.7108,16.9938)
(61.5071,17.3763)
(61.3035,18.7073)
(61.0998,19.2061)
(60.8961,19.3152)
(60.6925,19.4263)
(60.4888,19.5266)
(60.2851,19.8391)
(60.0815,20.1365)
(59.8778,20.3883)
(59.6741,20.7067)
(59.4705,21.5657)
(59.2668,21.6679)
(59.0631,22.1543)
(58.8595,22.2650)
(58.6558,22.5176)
(58.4521,22.6341)
(58.2485,22.7345)
(58.0448,23.1896)
(57.8411,23.2978)
(57.6375,23.4078)
(57.2301,23.5146)
(57.0265,24.5830)
(56.8228,25.4330)
(56.6191,25.5515)
(56.4155,25.6719)
(56.2118,25.7944)
(56.0081,25.8945)
(55.8045,25.9962)
(55.6008,26.6082)
(55.1935,26.7258)
(54.9898,27.8064)
(54.7862,28.1087)
(54.5825,28.2999)
(54.3788,28.4043)
(54.1752,29.0710)
(53.9715,29.3466)
(53.7678,29.7632)
(53.5642,29.9886)
(53.3605,31.0795)
(53.1568,31.5217)
(52.9532,33.4620)
(52.7495,33.5927)
(52.5458,33.8583)
(52.3422,33.9947)
(52.1385,34.1333)
(51.9348,34.3666)
(51.7312,34.6995)
(51.5275,34.8006)
(51.3238,34.9030)
(51.1202,35.1049)
(50.9165,35.2113)
(50.7128,35.5207)
(50.5092,36.0990)
(50.1018,36.2297)
(49.8982,36.3501)
(49.6945,36.7470)
(49.4908,37.2129)
(49.2872,37.7535)
(49.0835,37.8931)
(48.8798,38.0349)
(48.4725,37.8378)
(48.2688,37.9808)
(48.0652,38.1260)
(47.8615,38.5246)
(47.6578,39.0000)
(47.4542,39.3581)
(47.2505,39.5230)
(47.0468,40.1042)
(46.8432,40.7801)
(46.6395,40.8929)
(46.4358,41.0072)
(46.2322,41.1232)
(46.0285,41.0163)
(45.8248,41.1335)
(45.6212,41.0256)
(45.4175,41.1439)
(45.2138,41.2639)
(45.0102,41.3858)
(44.6029,41.2429)
(44.3992,41.3662)
(44.1955,41.2548)
(43.9919,41.3793)
(43.7882,41.5058)
(43.5845,41.3926)
(43.3809,41.9291)
(43.1772,42.1471)
(42.9735,42.2846)
(42.7699,42.7699)
(42.5662,42.9158)
(42.3625,43.1535)
(42.1589,43.3054)
(41.9552,43.4599)
(41.5479,43.5897)
(41.3442,43.7500)
(41.1405,43.6285)
(40.9369,43.5065)
(40.3259,43.3260)
(40.1222,43.7778)
(39.9185,43.9462)
(39.7149,43.8202)
(39.5112,44.3936)
(39.3075,44.8837)
(39.1039,45.2830)
(38.9002,45.4762)
(38.6965,45.8937)
(38.4929,46.0976)
(38.2892,46.6501)
(38.0855,47.1033)
(37.8819,47.2081)
(37.6782,47.3146)
(37.4745,47.4227)
(37.2709,48.1579)
(37.0672,48.6631)
(36.8635,48.5255)
(36.6599,48.7805)
(36.4562,49.0411)
(36.2525,48.9011)
(36.0489,49.3036)
(35.8452,49.1620)
(35.6415,49.0196)
(35.4379,48.8764)
(35.2342,48.7324)
(35.0305,48.5876)
(34.8269,48.4419)
(34.6232,48.2955)
(34.4196,48.4241)
(34.2159,48.6957)
(34.0122,48.9736)
(33.8086,49.4048)
(33.6049,49.2537)
(33.4012,49.1018)
(32.9939,48.9426)
(32.7902,49.5385)
(32.5866,49.3827)
(32.3829,49.2260)
(32.1792,49.0683)
(31.9756,48.9097)
(31.7719,48.7500)
(31.5682,48.8959)
(31.1609,48.7261)
(30.9572,48.8746)
(30.7536,49.6711)
(30.5499,49.5050)
(30.3462,49.3377)
(30.1426,49.4983)
(29.9389,49.8305)
(29.7352,49.6599)
(29.3279,49.4845)
(29.1242,49.3103)
(28.9206,49.4774)
(28.7169,49.6479)
(28.5132,49.4700)
(28.1059,49.2857)
(27.9022,49.4585)
(27.6986,49.2754)
(27.4949,49.6324)
(27.2912,49.4465)
(27.0876,49.2593)
(26.8839,50.1901)
(26.6802,50.0000)
(26.4766,50.3876)
(26.0692,50.1961)
(25.6619,50.0000)
(25.4582,50.2008)
(25.2546,50.4065)
(25.0509,50.6173)
(24.8473,50.4132)
(24.6436,50.8403)
(24.4399,50.6329)
(24.2363,50.4237)
(24.0326,50.8621)
(23.8289,51.3158)
(23.6253,51.1013)
(23.4216,51.3393)
(23.2179,51.1211)
(23.0143,50.9009)
(22.8106,50.6787)
(22.6069,51.1521)
(22.4033,50.9259)
(22.1996,50.6977)
(21.9959,51.4286)
(21.7923,51.1962)
(21.5886,51.4563)
(21.3849,51.7241)
(21.1813,52.0000)
(20.9776,51.7588)
(20.7739,51.5152)
(20.5703,51.2690)
(20.3666,51.0204)
(20.1629,50.7692)
(19.9593,51.0417)
(19.7556,51.3228)
(19.5519,51.0638)
(19.3483,51.3514)
(19.1446,51.0870)
(18.7373,50.8287)
(18.5336,50.5556)
(18.3299,50.2793)
(18.1263,50.0000)
(17.9226,49.7175)
(17.5153,49.4253)
(17.3116,49.1329)
(17.1079,48.8372)
(16.9043,48.5380)
(16.7006,48.2353)
(16.4969,47.9290)
(16.0896,47.5904)
(15.8859,47.2727)
(15.6823,47.5309)
(15.4786,47.7987)
(15.2749,47.4684)
(15.0713,47.1338)
(14.6640,46.7532)
(14.2566,46.3576)
(13.8493,45.9459)
(13.6456,45.5782)
(13.4420,45.8333)
(13.2383,46.4286)
(13.0346,46.7153)
(12.6273,46.2687)
(12.4236,45.8647)
(12.2200,46.1538)
(12.0163,45.7364)
(11.8126,45.3125)
(11.6090,44.8819)
(11.4053,44.4444)
(10.9980,43.9024)
(10.7943,43.8017)
(10.5906,43.6975)
(10.3870,43.2203)
(10.1833,42.7350)
(9.9796,42.9825)
(9.7760,42.4779)
(9.5723,41.9643)
(9.3686,41.4414)
(9.1650,42.0561)
(8.9613,43.5644)
(8.7576,43.4343)
(8.5540,43.2990)
(8.3503,43.1579)
(8.1466,43.0108)
(7.9430,42.3913)
(7.7393,42.2222)
(7.5356,42.0455)
(7.3320,41.3793)
(7.1283,40.6977)
(6.9246,40.0000)
(6.7210,39.7590)
(6.5173,40.0000)
(6.3136,40.2597)
(6.1100,40.0000)
(5.9063,40.8451)
(5.7026,40.5797)
(5.4990,40.2985)
(5.2953,40.0000)
(5.0916,39.6825)
(4.8880,40.0000)
(4.6843,38.9831)
(4.4807,41.5094)
(4.2770,41.1765)
(4.0733,40.0000)
(3.8697,38.7755)
(3.6660,37.5000)
(3.4623,39.5349)
(3.2587,39.0244)
(3.0550,50.0000)
(2.8513,48.2759)
(2.6477,52.0000)
(2.4440,52.1739)
(2.2403,50.0000)
(2.0367,52.6316)
(1.8330,81.8182)
(1.6293,88.8889)
(1.4257,87.5000)
(1.2220,85.7143)
(1.0183,83.3333)
(0.8147,100.0000)
(0.0,100.0000)};\addplot [draw=Cerulean, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,1.3067)
(99.7963,1.4068)
(98.9817,1.5068)
(98.7780,1.6069)
(98.3707,1.7070)
(97.7597,1.8070)
(96.9450,1.9071)
(96.1303,2.0071)
(95.1120,2.1071)
(92.8717,2.2072)
(90.8350,2.3072)
(90.0204,2.4073)
(87.7800,2.5074)
(84.7251,2.6075)
(81.0591,2.7077)
(76.7821,2.8078)
(70.8758,2.9080)
(67.0061,3.0081)
(66.1914,3.1083)
(50.9165,3.2084)
(45.0102,3.1057)
(41.9552,3.2057)
(37.2709,3.1033)
(28.3096,3.2035)
(28.1059,3.3038)
(25.2546,3.2000)
(21.1813,3.0925)
(15.8859,2.9760)
(14.0530,2.8738)
(13.6456,2.9738)
(13.2383,3.0747)
(11.6090,3.1755)
(11.4053,3.2768)
(10.9980,3.3771)
(10.7943,3.4777)
(9.5723,3.3547)
(9.3686,3.7037)
(8.9613,3.8062)
(8.7576,3.9091)
(8.5540,4.0115)
(7.7393,3.9054)
(7.3320,3.7500)
(7.1283,3.8976)
(6.9246,4.0964)
(6.7210,4.2581)
(6.5173,4.1505)
(6.3136,4.4097)
(5.9063,4.5101)
(5.7026,4.6129)
(5.4990,4.7203)
(5.2953,4.6018)
(5.0916,4.4803)
(4.8880,4.3400)
(4.6843,4.4402)
(4.4807,4.8140)
(4.2770,5.1597)
(4.0733,5.5556)
(3.8697,5.6716)
(3.6660,5.4381)
(3.4623,5.1672)
(3.2587,5.0000)
(3.0550,4.8232)
(2.8513,4.6358)
(2.6477,4.3189)
(2.4440,4.4280)
(2.2403,4.5455)
(2.0367,4.2373)
(1.8330,4.3478)
(1.6293,4.0609)
(1.4257,3.8043)
(1.2220,3.4483)
(1.0183,3.1250)
(0.8147,3.3613)
(0.6110,3.6585)
(0.4073,2.5641)
(0.2037,1.5873)
(0.0000,0.0000)
(0.0,0.0000)};\addlegendentry{GNN (BugLab + Real) (AP = 29.99)}
\addlegendentry{GNN (Only BugLab) (AP = 3.07)}


==> figures/rp/gnn/tex/gnn-synthetic-argument-swap.tex <==

\nextgroupplot[
	title={(a) Synthetic}
]
\addplot [draw=Peach, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.7046)
(98.7805,0.8046)
(94.3089,0.9046)
(89.0244,1.0046)
(85.3659,1.1047)
(82.1138,1.2047)
(77.6423,1.3048)
(74.3902,1.4049)
(69.5122,1.5049)
(69.1057,1.6255)
(66.2602,1.7256)
(64.2276,1.8257)
(59.7561,1.9258)
(55.6911,2.0260)
(52.8455,2.1263)
(49.5935,2.2263)
(45.1220,2.3266)
(44.7154,2.4592)
(40.2439,2.5595)
(39.8374,2.6602)
(37.8049,2.7605)
(32.5203,2.6552)
(30.8943,2.7556)
(28.4553,2.8560)
(28.0488,3.0572)
(27.6423,3.1584)
(26.0163,3.2587)
(25.6098,3.3600)
(23.9837,3.4604)
(23.5772,4.4241)
(23.1707,4.7619)
(21.9512,4.8649)
(21.5447,5.0669)
(20.7317,4.9515)
(19.9187,4.7665)
(19.5122,4.8682)
(19.1057,5.1762)
(18.6992,5.9202)
(18.2927,6.0241)
(17.4797,6.1254)
(17.0732,6.0086)
(16.2602,5.8394)
(15.8537,5.9724)
(15.4472,6.2500)
(14.6341,6.3604)
(14.2276,6.4695)
(13.8211,6.9672)
(13.4146,8.1281)
(12.6016,7.9082)
(12.1951,8.0214)
(11.7886,8.3095)
(11.3821,8.0692)
(10.9756,8.8525)
(10.5691,8.7248)
(10.1626,10.5485)
(9.7561,10.2128)
(9.3496,10.0437)
(8.9431,12.0879)
(8.5366,14.0940)
(8.1301,19.6078)
(7.7236,20.0000)
(7.3171,19.1489)
(6.9106,19.7674)
(6.5041,21.0526)
(6.0976,25.0000)
(5.6911,63.6364)
(5.2846,72.2222)
(4.8780,92.3077)
(4.4715,91.6667)
(4.0650,90.9091)
(3.6585,90.0000)
(3.2520,88.8889)
(2.8455,87.5000)
(2.4390,85.7143)
(2.0325,83.3333)
(1.6260,80.0000)
(1.2195,100.0000)
(0.0,100.0000)};\addplot [draw=Plum, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.5482)
(98.7805,0.6482)
(89.0244,0.7482)
(80.4878,0.8482)
(69.9187,0.9483)
(65.0407,1.0483)
(52.4390,1.1483)
(44.7154,1.2484)
(40.2439,1.3488)
(36.1789,1.4488)
(27.2358,1.5491)
(20.3252,1.6496)
(18.6992,1.7497)
(17.4797,1.8503)
(16.6667,1.9505)
(16.2602,2.1517)
(15.8537,2.2517)
(15.4472,2.6685)
(15.0407,3.1516)
(14.6341,3.2967)
(14.2276,3.5461)
(13.8211,3.7904)
(13.4146,3.8915)
(13.0081,4.0000)
(12.6016,4.1005)
(12.1951,4.2017)
(11.7886,4.3027)
(11.3821,4.4657)
(10.9756,5.4545)
(10.5691,5.5556)
(10.1626,5.6561)
(9.7561,5.4422)
(9.3496,5.8974)
(8.9431,5.7743)
(8.5366,6.8182)
(8.1301,8.4746)
(7.7236,8.2969)
(7.3171,7.8947)
(6.9106,10.1796)
(6.5041,12.0301)
(6.0976,11.5385)
(5.6911,37.8378)
(5.2846,46.4286)
(4.8780,50.0000)
(4.4715,52.3810)
(4.0650,66.6667)
(3.6585,90.0000)
(3.2520,88.8889)
(2.8455,87.5000)
(2.4390,85.7143)
(2.0325,83.3333)
(1.6260,100.0000)
(0.0,100.0000)};\addplot [draw=Cerulean, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.5961)
(89.8374,0.6961)
(73.5772,0.7961)
(64.6341,0.8961)
(56.9106,0.9962)
(32.9268,1.0962)
(28.0488,1.1963)
(26.8293,1.2964)
(24.7967,1.3965)
(23.9837,1.4967)
(19.9187,1.5971)
(18.6992,1.6974)
(17.4797,1.7977)
(16.6667,1.8981)
(16.2602,2.2818)
(15.8537,2.3824)
(15.0407,2.4832)
(14.2276,2.5849)
(13.8211,2.7961)
(13.0081,2.8986)
(12.6016,3.1633)
(12.1951,3.2644)
(11.7886,3.3682)
(11.3821,3.4696)
(10.9756,3.5714)
(10.5691,3.6723)
(10.1626,4.0064)
(9.7561,4.1096)
(9.3496,4.2831)
(8.9431,5.6410)
(8.5366,8.0460)
(8.1301,10.1010)
(7.7236,11.0465)
(6.9106,10.5590)
(6.5041,15.3846)
(6.0976,17.6471)
(5.6911,22.9508)
(5.2846,46.4286)
(4.8780,44.4444)
(4.4715,42.3077)
(4.0650,40.0000)
(3.6585,60.0000)
(3.2520,57.1429)
(2.8455,53.8462)
(2.4390,54.5455)
(2.0325,55.5556)
(1.6260,80.0000)
(1.2195,100.0000)
(0.0,100.0000)};\addlegendentry{Our Model  (Synthetic + Real) (AP = 8.49)}
\addlegendentry{GNN (Synthetic + Real) (AP = 6.44)}
\addlegendentry{GNN (Only Synthetic) (AP = 5.42)}


==> figures/rp/gnn/tex/gnn-synthetic-var-misuse.tex <==

\nextgroupplot[
	title={(a) \varmisuse{} (Synthetic)}
]
\addplot [draw=Peach, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.9871)
(99.1071,1.0871)
(98.5119,1.1871)
(97.0238,1.2872)
(96.4286,1.3872)
(95.8333,1.4872)
(94.3452,1.5873)
(93.4524,1.6874)
(92.8571,1.7875)
(92.2619,1.8875)
(91.3690,1.9876)
(91.0714,2.0876)
(90.7738,2.2206)
(88.9881,2.3207)
(87.5000,2.4207)
(86.6071,2.5208)
(85.1190,2.6212)
(83.6310,2.7213)
(83.3333,2.8214)
(83.0357,2.9215)
(81.2500,3.0216)
(80.9524,3.1218)
(80.6548,3.2220)
(79.1667,3.3221)
(77.9762,3.4222)
(77.3810,3.5230)
(77.0833,3.6234)
(76.7857,3.7235)
(76.1905,3.8237)
(74.4048,3.9240)
(74.1071,4.0246)
(73.5119,4.1249)
(72.9167,4.2256)
(72.6190,4.3262)
(71.4286,4.4264)
(70.8333,4.5264)
(70.2381,4.6275)
(69.0476,4.7279)
(68.7500,4.8316)
(66.6667,4.9317)
(66.3690,5.0327)
(65.7738,5.1336)
(65.4762,5.2344)
(65.1786,5.3808)
(64.5833,5.4812)
(64.2857,5.6265)
(63.3929,5.7273)
(63.0952,5.8274)
(62.7976,5.9605)
(61.9048,6.0606)
(61.6071,6.1607)
(60.1190,6.2616)
(59.2262,6.3619)
(58.9286,6.4621)
(58.6310,6.6130)
(57.4405,6.7130)
(57.1429,6.8133)
(55.9524,6.9143)
(54.7619,7.0149)
(54.1667,7.1149)
(53.5714,7.2173)
(53.2738,7.3181)
(52.9762,7.4947)
(52.6786,7.5966)
(52.3810,7.6990)
(52.0833,7.8021)
(51.7857,8.0184)
(51.4881,8.1221)
(49.1071,8.2253)
(47.9167,8.3290)
(47.6190,8.4971)
(47.3214,8.5992)
(47.0238,9.0909)
(46.7262,9.1920)
(46.4286,9.5588)
(46.1310,9.6633)
(45.8333,9.7654)
(45.2381,9.8701)
(44.6429,9.9734)
(44.3452,10.1017)
(44.0476,10.2069)
(43.1548,10.3129)
(42.8571,10.4197)
(42.5595,10.5769)
(41.9643,10.4755)
(41.3690,10.5784)
(40.7738,10.6864)
(40.4762,10.7937)
(39.8810,10.8943)
(39.2857,11.0000)
(38.6905,11.1016)
(37.5000,11.2100)
(37.2024,11.3740)
(36.9048,11.4815)
(36.6071,11.5819)
(36.0119,11.4801)
(35.7143,11.6732)
(35.4167,11.7822)
(35.1190,12.0041)
(34.8214,12.2642)
(34.5238,12.5405)
(34.2262,12.6513)
(33.9286,12.7517)
(32.7381,12.8655)
(32.4405,13.0539)
(32.1429,14.5749)
(31.8452,14.6776)
(31.2500,14.5028)
(30.6548,14.6099)
(30.3571,14.7186)
(30.0595,15.1880)
(29.7619,15.3374)
(29.4643,15.4446)
(29.1667,16.3606)
(28.8690,16.6381)
(28.5714,16.8717)
(27.9762,16.7260)
(27.6786,16.6071)
(27.3810,16.7273)
(27.0833,16.8519)
(26.7857,17.7515)
(26.4881,18.1633)
(26.1905,20.1373)
(25.8929,21.3759)
(25.5952,21.1823)
(25.2976,22.7273)
(25.0000,22.5201)
(24.7024,23.6467)
(24.4048,24.9240)
(24.1071,25.5521)
(23.8095,25.9740)
(23.5119,26.8707)
(23.2143,26.7123)
(22.9167,26.5517)
(22.6190,27.9412)
(22.3214,29.6443)
(22.0238,29.4821)
(21.7262,29.9180)
(21.4286,30.1255)
(21.1310,29.9578)
(20.8333,29.7872)
(20.5357,30.0000)
(20.2381,32.5359)
(19.9405,34.5361)
(19.6429,34.3750)
(19.3452,34.0314)
(19.0476,34.9727)
(18.7500,41.4474)
(18.4524,42.4658)
(18.1548,46.2121)
(17.8571,46.5116)
(17.5595,46.0938)
(17.2619,46.7742)
(16.9643,46.3415)
(16.6667,46.6667)
(16.3690,47.0085)
(16.0714,47.3684)
(15.4762,46.8468)
(15.1786,47.2222)
(14.8810,48.5437)
(14.5833,49.4949)
(14.2857,50.0000)
(13.9881,57.3171)
(13.6905,56.7901)
(13.3929,64.2857)
(13.0952,65.6716)
(12.7976,65.1515)
(12.5000,64.6154)
(12.2024,64.0625)
(11.9048,66.6667)
(11.6071,66.1017)
(11.3095,65.5172)
(11.0119,66.0714)
(10.7143,65.4545)
(10.4167,64.8148)
(10.1190,65.3846)
(9.8214,67.3469)
(9.5238,68.0851)
(9.2262,68.8889)
(8.9286,68.1818)
(8.6310,67.4419)
(8.3333,71.7949)
(8.0357,77.1429)
(7.7381,78.7879)
(7.4405,86.2069)
(7.1429,85.7143)
(6.8452,88.4615)
(6.5476,88.0000)
(6.2500,91.3043)
(5.9524,95.2381)
(5.6548,95.0000)
(5.3571,94.7368)
(5.0595,94.4444)
(4.7619,94.1176)
(4.4643,93.7500)
(4.1667,93.3333)
(3.8690,92.8571)
(3.5714,92.3077)
(3.2738,91.6667)
(2.9762,90.9091)
(2.6786,90.0000)
(2.3810,100.0000)
(0.0,100.0000)};\addplot [draw=Plum, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.7407)
(99.4048,0.8408)
(98.8095,0.9408)
(97.9167,1.0408)
(95.5357,1.1408)
(94.3452,1.2409)
(92.8571,1.3410)
(91.6667,1.4410)
(88.3929,1.5411)
(86.6071,1.6411)
(83.6310,1.7412)
(83.3333,1.8413)
(80.6548,1.9413)
(78.2738,2.0413)
(69.9405,2.1414)
(67.5595,2.2415)
(62.5000,2.3417)
(60.7143,2.4419)
(50.8929,2.5420)
(48.8095,2.6422)
(44.0476,2.7423)
(41.6667,2.8426)
(40.7738,2.9431)
(35.4167,3.0435)
(34.2262,3.1438)
(28.5714,3.0179)
(25.2976,3.1181)
(24.7024,3.2183)
(22.6190,3.0945)
(19.6429,3.1946)
(19.3452,3.5852)
(19.0476,3.6866)
(18.7500,3.7883)
(18.4524,3.8896)
(17.2619,3.7371)
(16.6667,3.8382)
(15.7738,3.9405)
(14.5833,3.8043)
(14.2857,3.9056)
(13.9881,4.0068)
(13.3929,4.1096)
(12.7976,3.9595)
(12.5000,4.0619)
(12.2024,4.4662)
(11.6071,4.3527)
(11.3095,4.7679)
(10.7143,4.8714)
(10.4167,4.9716)
(10.1190,5.0746)
(9.5238,4.9155)
(9.2262,5.0162)
(8.6310,4.8739)
(8.3333,4.9822)
(8.0357,4.8214)
(7.7381,4.9242)
(7.4405,5.0302)
(7.1429,5.2061)
(6.8452,5.3488)
(6.5476,6.1281)
(6.2500,6.0000)
(5.9524,6.1162)
(5.6548,6.2295)
(5.3571,6.3380)
(5.0595,6.6667)
(4.7619,6.2992)
(4.4643,6.0484)
(4.1667,6.1674)
(3.8690,6.3107)
(3.5714,6.4171)
(3.2738,7.0513)
(2.9762,7.1942)
(2.6786,8.8235)
(2.3810,8.9888)
(2.0833,10.9375)
(1.7857,26.0870)
(1.4881,31.2500)
(1.1905,28.5714)
(0.8929,100.0000)
(0.0,100.0000)};\addplot [draw=Cerulean, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.7561)
(99.1071,0.8561)
(95.5357,0.9561)
(92.2619,1.0561)
(87.5000,1.1562)
(77.0833,1.2562)
(61.0119,1.3563)
(45.5357,1.4563)
(42.8571,1.5564)
(30.9524,1.6566)
(27.9762,1.7567)
(20.5357,1.6425)
(18.4524,1.7426)
(12.5000,1.8429)
(11.6071,1.9432)
(11.3095,2.0441)
(10.4167,1.9305)
(10.1190,2.0311)
(9.8214,2.1318)
(9.5238,2.3088)
(7.4405,2.2007)
(7.1429,2.5184)
(6.5476,2.3732)
(6.2500,2.7778)
(5.9524,3.0211)
(5.6548,3.4234)
(5.3571,3.6735)
(5.0595,3.5417)
(4.7619,3.4261)
(4.4643,3.6496)
(4.1667,3.4314)
(3.5714,3.1579)
(3.2738,3.3033)
(2.9762,4.4248)
(2.6786,6.1644)
(2.3810,5.7554)
(2.0833,15.2174)
(1.7857,15.0000)
(1.4881,15.1515)
(1.1905,19.0476)
(0.8929,17.6471)
(0.5952,16.6667)
(0.2976,50.0000)
(0.0000,100.0000)
(0.0,100.0000)};\addlegendentry{Our Model  (Synthetic + Real) (AP = 20.96)}
\addlegendentry{GNN (Synthetic + Real) (AP = 4.28)}
\addlegendentry{GNN (Only Synthetic) (AP = 2.38)}


==> figures/rp/gnn/tex/gnn-synthetic-wrong-binary-operator.tex <==

\nextgroupplot[
	title={(b) \wrongbinop{} (Synthetic)}
]
\addplot [draw=Peach, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,1.8454)
(99.5927,1.9454)
(99.3890,2.3306)
(98.9817,2.4306)
(98.3707,2.5307)
(97.7597,2.6307)
(97.5560,2.7637)
(97.3523,2.8638)
(97.1487,2.9640)
(96.5377,3.0642)
(96.3340,3.1643)
(96.1303,3.2644)
(95.9267,3.3645)
(95.7230,3.4645)
(95.3157,3.5646)
(95.1120,3.6648)
(94.9084,3.7650)
(94.5010,3.8651)
(94.2974,3.9651)
(93.6864,4.0654)
(93.4827,4.2690)
(93.0754,4.3690)
(92.8717,4.5041)
(92.4644,4.6045)
(92.2607,4.7330)
(91.6497,4.8335)
(91.0387,4.9338)
(90.8350,5.1602)
(90.6314,5.2607)
(90.4277,5.3610)
(90.2240,5.4610)
(89.8167,5.5612)
(89.6130,5.8737)
(89.4094,6.0938)
(89.2057,6.2022)
(88.5947,6.3025)
(88.3910,6.4031)
(87.9837,6.5031)
(87.1690,6.6039)
(86.9654,6.7043)
(86.7617,6.8062)
(86.5580,6.9072)
(86.3544,7.0083)
(86.1507,7.1092)
(85.7434,7.2101)
(85.5397,7.5080)
(85.3360,7.6460)
(84.9287,7.7466)
(84.7251,7.9163)
(84.3177,8.0170)
(84.1141,8.1171)
(83.9104,8.2186)
(83.7067,8.4900)
(83.5031,8.9053)
(83.2994,9.1478)
(83.0957,9.3685)
(82.8921,9.4695)
(82.6884,9.9632)
(82.4847,10.0646)
(82.2811,10.6288)
(82.0774,10.8333)
(81.8737,10.9656)
(80.2444,11.0674)
(80.0407,11.1679)
(79.8371,11.2871)
(79.6334,11.4461)
(79.4297,11.5556)
(78.8187,11.6566)
(78.6151,11.7575)
(78.4114,11.8608)
(78.2077,12.2021)
(77.3931,12.3057)
(77.1894,12.4059)
(76.9857,12.5083)
(76.7821,12.7797)
(76.3747,12.8822)
(76.1711,12.9861)
(75.9674,13.0969)
(75.7637,13.2009)
(75.5601,13.3935)
(75.3564,13.4938)
(75.1527,13.7635)
(74.3381,13.8678)
(74.1344,14.1524)
(73.9308,14.2577)
(73.7271,14.5090)
(73.5234,14.6569)
(73.3198,14.7601)
(73.1161,15.3419)
(72.7088,15.4479)
(72.5051,15.5526)
(72.3014,15.7358)
(72.0978,15.8531)
(71.8941,15.9584)
(71.6904,16.0951)
(71.4868,16.3104)
(71.2831,16.4706)
(71.0794,16.6032)
(70.8758,16.8197)
(70.6721,17.0265)
(70.4684,17.3173)
(70.2648,17.4242)
(70.0611,17.5331)
(69.8574,17.9769)
(69.6538,18.4566)
(69.4501,18.8086)
(69.2464,19.0157)
(69.0428,19.6979)
(68.8391,20.3737)
(68.6354,20.7640)
(68.4318,20.9738)
(68.2281,21.1356)
(68.0244,21.3010)
(67.8208,22.0093)
(67.6171,22.1629)
(67.4134,23.1631)
(67.2098,23.4209)
(67.0061,23.5336)
(66.8024,24.3685)
(66.5988,24.5495)
(66.3951,25.4887)
(66.1914,25.6917)
(65.9878,26.0450)
(65.7841,26.3458)
(65.5804,26.4585)
(65.3768,27.5064)
(65.1731,27.6339)
(64.9695,27.7391)
(64.7658,27.9683)
(64.5621,28.2028)
(64.1548,28.0999)
(63.9511,28.3906)
(63.7475,28.5064)
(63.5438,28.9157)
(63.3401,30.2824)
(63.1365,30.4519)
(62.9328,30.5638)
(62.7291,30.7692)
(62.5255,31.1992)
(62.3218,31.3846)
(61.9145,31.5026)
(61.7108,32.3028)
(61.5071,32.4034)
(61.3035,32.9322)
(61.0998,33.0396)
(60.8961,33.2592)
(60.6925,33.3707)
(60.4888,33.7117)
(60.2851,33.9839)
(60.0815,34.7059)
(59.8778,34.8754)
(59.6741,35.0060)
(59.4705,35.1384)
(59.2668,35.2727)
(59.0631,36.7089)
(58.8595,37.0988)
(58.6558,37.2574)
(58.4521,37.3698)
(58.2485,37.4836)
(58.0448,38.5656)
(57.8411,39.0110)
(57.6375,39.3056)
(57.4338,40.2282)
(57.2301,40.7837)
(57.0265,41.1160)
(56.4155,41.2202)
(56.2118,41.3793)
(56.0081,41.5408)
(55.8045,41.8321)
(55.6008,42.1296)
(55.3971,42.2360)
(55.1935,42.3438)
(54.9898,42.6540)
(54.3788,42.5159)
(54.1752,42.8341)
(53.9715,43.3715)
(53.7678,43.4926)
(53.5642,43.7604)
(53.1568,43.8655)
(52.5458,43.7288)
(52.3422,44.9301)
(52.1385,46.4610)
(51.7312,46.3504)
(51.5275,46.6790)
(51.3238,46.9274)
(51.1202,47.0919)
(50.7128,46.9811)
(50.5092,47.2381)
(50.3055,47.1374)
(49.8982,47.2973)
(49.6945,47.1954)
(49.4908,47.0930)
(49.2872,47.7318)
(48.8798,47.9042)
(48.6762,48.0885)
(48.4725,47.9839)
(48.2688,48.1707)
(48.0652,48.3607)
(47.8615,48.2546)
(47.6578,48.1481)
(47.4542,48.3402)
(47.2505,49.5726)
(47.0468,49.6774)
(46.8432,49.8915)
(46.6395,50.0000)
(46.4358,50.1099)
(46.0285,50.0000)
(45.8248,49.8891)
(45.6212,50.0000)
(45.4175,50.9132)
(45.2138,51.1521)
(45.0102,51.2761)
(44.8065,51.4019)
(44.6029,51.5294)
(44.3992,51.6588)
(44.1955,51.5439)
(43.9919,52.3002)
(43.7882,52.4390)
(43.5845,52.5799)
(43.3809,52.7228)
(43.1772,52.6055)
(42.9735,53.0151)
(42.7699,53.2995)
(42.5662,53.1807)
(42.1589,53.0769)
(41.9552,53.2300)
(41.7515,53.3854)
(41.5479,53.2637)
(41.3442,53.1414)
(41.1405,53.2982)
(40.9369,53.7433)
(40.7332,54.3478)
(40.5295,54.5205)
(40.1222,54.4199)
(39.9185,54.5961)
(39.7149,54.4693)
(39.3075,54.3662)
(39.1039,54.2373)
(38.9002,54.8851)
(38.6965,54.7550)
(38.4929,54.9419)
(38.2892,54.8105)
(38.0855,54.6784)
(37.8819,54.5455)
(37.6782,54.7337)
(37.4745,54.9254)
(37.2709,55.1205)
(37.0672,56.8750)
(36.8635,57.0978)
(36.6599,57.3248)
(35.8452,57.1429)
(35.6415,57.5658)
(35.2342,57.6667)
(35.0305,57.9125)
(34.8269,57.7703)
(34.6232,58.0205)
(34.4196,57.8767)
(34.2159,58.9474)
(34.0122,58.8028)
(33.8086,58.6572)
(33.6049,58.9286)
(33.4012,59.2058)
(33.1976,59.0580)
(32.9939,59.3407)
(32.7902,59.1912)
(32.5866,59.0406)
(32.1792,59.1760)
(31.9756,59.4697)
(31.7719,59.3156)
(31.5682,60.3113)
(31.3646,60.6299)
(31.1609,60.4743)
(30.9572,60.8000)
(30.7536,60.6426)
(30.5499,60.9756)
(30.3462,61.5702)
(30.1426,61.4108)
(29.9389,61.7647)
(29.7352,62.1277)
(29.5316,61.9658)
(29.3279,62.0690)
(29.1242,62.1739)
(28.9206,62.0087)
(28.7169,61.8421)
(28.5132,62.2222)
(28.3096,62.3318)
(28.1059,62.1622)
(27.9022,61.9910)
(27.6986,61.8182)
(27.4949,61.6438)
(27.2912,61.7512)
(27.0876,61.8605)
(26.8839,61.6822)
(26.6802,61.5023)
(26.4766,61.9048)
(26.2729,61.7225)
(26.0692,62.4390)
(25.8656,62.8713)
(25.6619,63.0000)
(25.4582,62.8141)
(25.2546,62.9442)
(25.0509,62.7551)
(24.8473,62.8866)
(24.6436,64.3617)
(24.4399,64.5161)
(24.2363,65.7459)
(24.0326,65.9218)
(23.8289,65.7303)
(23.6253,65.9091)
(23.4216,65.7143)
(23.2179,66.2791)
(23.0143,67.6647)
(22.8106,67.4699)
(22.6069,67.6829)
(22.4033,67.9012)
(22.1996,68.5535)
(21.9959,68.7898)
(21.7923,68.5897)
(21.5886,68.3871)
(21.3849,68.1818)
(21.1813,68.4211)
(20.9776,69.1275)
(20.7739,68.9189)
(20.5703,69.1781)
(20.3666,68.9655)
(20.1629,68.7500)
(19.9593,69.0141)
(19.7556,68.7943)
(19.5519,70.5882)
(19.3483,70.8955)
(19.1446,71.2121)
(18.9409,70.9924)
(18.7373,70.7692)
(18.5336,70.5426)
(18.3299,70.3125)
(18.1263,70.0787)
(17.9226,69.8413)
(17.7189,69.6000)
(17.5153,69.9187)
(17.3116,69.6721)
(17.1079,69.4215)
(16.9043,69.1667)
(16.7006,68.9076)
(16.4969,68.6441)
(16.2933,68.3761)
(16.0896,68.1034)
(15.8859,67.8261)
(15.6823,67.5439)
(15.4786,68.4685)
(15.2749,68.1818)
(15.0713,68.5185)
(14.8676,68.2243)
(14.6640,67.9245)
(14.4603,67.6190)
(14.2566,67.3077)
(14.0530,67.6471)
(13.8493,67.3267)
(13.6456,67.0000)
(13.4420,66.6667)
(13.2383,66.3265)
(13.0346,66.6667)
(12.8310,66.3158)
(12.6273,65.9574)
(12.4236,65.5914)
(12.2200,65.2174)
(12.0163,65.5556)
(11.8126,65.1685)
(11.6090,64.7727)
(11.4053,65.1163)
(11.2016,64.7059)
(10.9980,64.2857)
(10.7943,63.8554)
(10.5906,63.4146)
(10.3870,64.5570)
(10.1833,64.1026)
(9.9796,63.6364)
(9.7760,63.1579)
(9.5723,62.6667)
(9.3686,62.1622)
(9.1650,61.6438)
(8.9613,61.1111)
(8.7576,61.4286)
(8.5540,60.8696)
(8.3503,60.2941)
(8.1466,59.7015)
(7.9430,60.9375)
(7.7393,60.3175)
(7.5356,59.6774)
(7.3320,59.0164)
(7.1283,59.3220)
(6.9246,58.6207)
(6.7210,57.8947)
(6.5173,60.3774)
(6.3136,59.6154)
(6.1100,58.8235)
(5.9063,58.0000)
(5.7026,57.1429)
(5.4990,56.2500)
(5.2953,55.3191)
(5.0916,59.5238)
(4.8880,58.5366)
(4.6843,57.5000)
(4.4807,57.8947)
(4.2770,56.7568)
(4.0733,58.8235)
(3.8697,57.5758)
(3.6660,58.0645)
(3.4623,56.6667)
(3.2587,59.2593)
(3.0550,60.0000)
(2.8513,58.3333)
(2.6477,56.5217)
(2.4440,60.0000)
(2.2403,57.8947)
(2.0367,55.5556)
(1.8330,52.9412)
(1.6293,57.1429)
(1.4257,53.8462)
(1.2220,60.0000)
(1.0183,55.5556)
(0.8147,50.0000)
(0.6110,60.0000)
(0.4073,66.6667)
(0.2037,50.0000)
(0.0000,100.0000)
(0.0,100.0000)};\addplot [draw=Plum, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,1.4833)
(98.9817,1.5834)
(98.5743,1.6835)
(98.1670,1.7835)
(97.5560,1.8836)
(96.5377,1.9837)
(96.3340,2.1710)
(95.3157,2.2711)
(94.9084,2.3711)
(93.8900,2.4712)
(93.6864,2.5714)
(93.4827,2.6716)
(93.0754,2.7717)
(92.0570,2.8720)
(91.4460,2.9721)
(91.2424,3.0723)
(91.0387,3.1945)
(90.2240,3.2947)
(90.0204,3.3948)
(89.8167,3.4950)
(89.2057,3.5952)
(88.3910,3.6952)
(87.9837,3.7955)
(87.5764,3.8960)
(87.3727,3.9963)
(86.1507,4.0965)
(85.7434,4.1966)
(84.7251,4.2966)
(84.5214,4.4380)
(83.7067,4.5384)
(83.5031,4.6385)
(83.2994,4.7387)
(83.0957,4.9163)
(82.4847,5.0167)
(82.2811,5.1968)
(82.0774,5.3698)
(81.6701,5.4699)
(81.4664,5.5703)
(81.2627,5.6708)
(80.8554,5.7712)
(80.6517,5.8719)
(80.4481,5.9722)
(79.8371,6.0728)
(79.6334,6.2341)
(79.4297,6.3590)
(79.2261,6.4682)
(78.8187,6.5693)
(78.6151,6.6886)
(78.2077,6.7893)
(78.0041,6.9084)
(77.8004,7.1389)
(77.5967,7.2392)
(76.7821,7.3403)
(76.5784,7.5426)
(76.3747,7.6437)
(75.7637,7.7452)
(74.9491,7.8465)
(74.5418,7.9479)
(74.3381,8.1401)
(74.1344,8.2409)
(73.7271,8.3410)
(73.5234,8.5041)
(73.3198,8.6042)
(73.1161,8.9237)
(72.9124,9.1141)
(72.7088,9.2153)
(71.8941,9.3164)
(71.6904,9.4168)
(71.4868,9.5174)
(71.2831,9.6180)
(70.8758,9.7207)
(69.8574,9.8225)
(69.4501,9.9243)
(69.2464,10.3343)
(69.0428,10.4986)
(68.4318,10.5994)
(68.2281,10.7372)
(67.6171,10.8390)
(67.2098,10.9416)
(67.0061,11.3723)
(66.8024,11.4725)
(66.5988,11.5752)
(66.3951,11.7988)
(65.9878,11.9030)
(65.7841,12.0433)
(65.5804,12.5341)
(65.3768,12.6378)
(65.1731,12.8669)
(64.9695,12.9675)
(64.1548,13.0705)
(63.9511,13.2489)
(63.7475,13.4335)
(63.5438,13.5652)
(63.3401,13.9212)
(63.1365,14.1423)
(62.9328,15.0953)
(62.7291,15.3158)
(62.5255,15.7922)
(62.1181,15.8937)
(61.9145,18.9408)
(61.7108,19.0446)
(61.5071,19.3218)
(61.3035,19.4319)
(61.0998,20.1207)
(60.8961,20.2300)
(60.6925,20.3552)
(60.4888,20.7692)
(60.2851,20.9632)
(60.0815,21.0714)
(59.8778,21.2581)
(59.6741,21.3713)
(59.4705,21.5498)
(58.8595,21.4074)
(58.6558,21.8017)
(58.4521,22.5275)
(58.2485,22.7888)
(58.0448,23.3607)
(57.8411,23.6273)
(57.6375,23.9020)
(57.4338,24.3734)
(57.2301,25.2018)
(57.0265,25.7590)
(56.8228,26.2712)
(56.6191,27.0428)
(56.4155,27.3715)
(56.2118,27.5174)
(56.0081,27.6382)
(55.8045,27.7609)
(55.3971,27.8689)
(55.1935,28.0829)
(54.9898,28.1837)
(54.7862,28.3755)
(54.5825,28.4803)
(54.1752,28.6022)
(53.9715,31.7746)
(53.7678,31.8841)
(53.3605,31.7576)
(53.1568,31.8681)
(52.9532,31.9803)
(52.7495,32.2139)
(52.5458,32.8662)
(52.3422,35.9944)
(52.1385,36.1072)
(51.9348,36.2216)
(51.7312,36.3376)
(51.5275,36.8805)
(51.3238,37.5559)
(51.1202,37.6877)
(50.9165,37.8215)
(50.7128,37.9573)
(50.5092,38.0952)
(50.1018,38.1988)
(49.8982,38.4013)
(49.6945,38.8535)
(49.2872,38.9694)
(49.0835,39.1234)
(48.4725,39.0164)
(48.2688,39.3688)
(47.6578,39.2617)
(47.0468,39.1525)
(46.8432,39.3162)
(46.6395,39.8261)
(46.4358,40.0000)
(46.2322,40.1060)
(46.0285,40.0000)
(45.8248,40.1070)
(45.6212,40.0000)
(45.4175,40.1079)
(45.2138,40.0000)
(45.0102,39.8917)
(44.8065,40.1460)
(44.6029,40.0366)
(44.3992,40.8240)
(44.1955,40.9434)
(43.9919,40.8318)
(43.7882,40.9524)
(43.5845,40.8397)
(43.3809,40.7266)
(43.1772,40.8478)
(42.9735,41.1306)
(42.5662,40.9804)
(42.3625,41.4343)
(42.1589,41.3174)
(41.9552,41.4487)
(41.7515,41.5822)
(41.5479,41.7178)
(41.3442,41.9421)
(41.1405,41.8219)
(40.5295,41.6318)
(40.3259,41.5094)
(40.1222,41.3866)
(39.7149,41.2262)
(39.5112,41.1017)
(39.3075,40.9766)
(38.9002,40.8120)
(38.6965,40.6852)
(38.4929,40.8207)
(38.0855,40.6522)
(37.8819,40.7895)
(37.6782,40.6593)
(37.4745,40.7982)
(37.2709,40.6667)
(37.0672,40.5345)
(36.8635,40.7658)
(36.6599,40.6321)
(36.4562,40.7745)
(36.2525,40.6393)
(36.0489,40.5034)
(35.6415,40.6977)
(35.4379,40.8451)
(35.2342,41.0926)
(35.0305,40.9524)
(34.8269,41.1058)
(34.6232,41.2621)
(34.4196,41.1192)
(34.2159,40.9756)
(34.0122,40.8313)
(33.4012,40.5941)
(33.1976,40.9548)
(32.9939,40.8060)
(32.7902,40.6566)
(32.5866,40.8163)
(32.3829,41.0853)
(32.1792,40.9326)
(31.7719,41.0526)
(31.5682,41.2234)
(31.3646,41.0667)
(31.1609,40.9091)
(30.9572,40.7507)
(30.7536,40.5914)
(30.5499,40.9836)
(30.3462,40.8219)
(29.9389,40.7202)
(29.7352,40.8964)
(29.5316,41.0765)
(29.3279,40.9091)
(29.1242,41.0920)
(28.9206,40.9222)
(28.7169,40.7514)
(28.3096,40.5248)
(28.1059,40.3509)
(27.9022,40.1760)
(27.6986,40.0000)
(27.4949,39.8230)
(27.2912,39.6450)
(27.0876,39.4659)
(26.6802,39.2216)
(26.4766,39.0390)
(26.2729,38.8554)
(25.8656,38.7195)
(25.4582,38.5802)
(25.2546,38.3901)
(25.0509,38.1988)
(24.8473,38.0062)
(24.6436,37.8125)
(24.4399,37.6176)
(24.2363,37.7778)
(24.0326,37.5796)
(23.8289,37.7419)
(23.6253,37.9085)
(23.4216,37.7049)
(23.2179,37.8738)
(23.0143,38.0471)
(22.6069,37.8840)
(22.4033,38.0623)
(22.1996,38.2456)
(21.9959,38.4342)
(21.7923,38.7681)
(21.3849,38.6029)
(20.9776,38.4328)
(20.7739,38.2022)
(20.3666,37.8788)
(20.1629,37.6426)
(19.9593,37.8378)
(19.7556,38.0392)
(19.5519,38.2470)
(19.3483,38.0000)
(19.1446,38.3673)
(18.9409,38.1148)
(18.5336,37.9167)
(18.3299,37.8151)
(18.1263,38.0342)
(17.9226,38.2609)
(17.7189,38.6667)
(17.5153,39.8148)
(17.3116,40.4762)
(17.1079,40.1914)
(16.9043,41.0891)
(16.7006,41.8367)
(16.4969,41.9689)
(16.2933,41.6667)
(16.0896,41.7989)
(15.8859,41.9355)
(15.4786,41.5301)
(15.0713,41.1111)
(14.8676,41.4773)
(14.6640,41.6185)
(14.4603,41.7647)
(14.2566,41.4201)
(14.0530,41.3174)
(13.8493,40.9639)
(13.6456,40.8537)
(13.4420,40.4908)
(13.2383,40.1235)
(13.0346,39.7516)
(12.8310,39.6226)
(12.6273,39.4904)
(12.4236,39.1026)
(12.2200,39.7351)
(12.0163,39.3333)
(11.8126,38.9262)
(11.6090,38.5135)
(11.4053,38.6207)
(11.2016,38.1944)
(10.9980,37.7622)
(10.7943,37.3239)
(10.5906,37.1429)
(10.3870,36.6906)
(10.1833,37.0370)
(9.9796,37.9845)
(9.7760,37.5000)
(9.5723,37.3016)
(9.3686,36.8000)
(8.9613,36.3636)
(8.7576,36.7521)
(8.5540,36.2069)
(8.3503,37.6147)
(8.1466,39.2157)
(7.9430,39.7959)
(7.7393,39.1753)
(7.5356,38.5417)
(7.3320,37.8947)
(7.1283,38.4615)
(6.9246,37.7778)
(6.7210,37.9310)
(6.5173,37.6471)
(6.3136,37.3494)
(6.1100,36.5854)
(5.9063,36.2500)
(5.7026,35.4430)
(5.2953,34.6667)
(5.0916,35.2113)
(4.8880,34.2857)
(4.6843,33.3333)
(4.2770,32.3077)
(4.0733,36.3636)
(3.8697,35.8491)
(3.6660,34.6154)
(3.4623,34.0000)
(3.2587,32.6531)
(3.0550,34.0909)
(2.8513,32.5581)
(2.6477,30.9524)
(2.4440,30.0000)
(2.2403,39.2857)
(2.0367,37.0370)
(1.8330,34.6154)
(1.6293,36.3636)
(1.4257,38.8889)
(1.2220,40.0000)
(1.0183,38.4615)
(0.8147,66.6667)
(0.6110,60.0000)
(0.4073,50.0000)
(0.0000,0.0000)
(0.0,0.0000)};\addplot [draw=Cerulean, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,1.3044)
(99.5927,1.4044)
(99.3890,1.5044)
(99.1853,1.6045)
(98.7780,1.7045)
(97.7597,1.8045)
(95.9267,1.9046)
(94.5010,2.0046)
(92.2607,2.1046)
(91.0387,2.2047)
(90.2240,2.3048)
(88.5947,2.4048)
(87.3727,2.5048)
(86.3544,2.6049)
(84.9287,2.7050)
(84.7251,2.8061)
(82.8921,2.9061)
(81.6701,3.0062)
(81.4664,3.1066)
(79.8371,3.2068)
(79.4297,3.3070)
(78.8187,3.4073)
(77.5967,3.5073)
(74.1344,3.6075)
(73.1161,3.7079)
(72.7088,3.8080)
(71.0794,3.9082)
(70.4684,4.0083)
(70.2648,4.1086)
(69.8574,4.2091)
(69.6538,4.3095)
(68.8391,4.4097)
(68.6354,4.5102)
(68.4318,4.6103)
(66.3951,4.7110)
(65.7841,4.8116)
(65.3768,4.9120)
(63.5438,5.0120)
(62.3218,5.1128)
(60.8961,5.2136)
(60.6925,5.3138)
(60.2851,5.4143)
(58.8595,5.5153)
(56.6191,5.6162)
(53.5642,5.5090)
(44.6029,5.6096)
(35.2342,5.7115)
(34.2159,5.8131)
(32.5866,5.9150)
(32.3829,6.0159)
(31.5682,6.1168)
(31.3646,6.2172)
(30.7536,6.3180)
(28.9206,6.4195)
(27.6986,6.5197)
(27.4949,6.6209)
(27.2912,6.7235)
(26.0692,6.6082)
(25.8656,6.7410)
(25.4582,6.8418)
(25.2546,6.9429)
(23.2179,6.8386)
(22.4033,6.9401)
(21.9959,6.8225)
(21.7923,6.9256)
(20.7739,6.8227)
(20.5703,6.9416)
(19.3483,6.7906)
(18.9409,6.6714)
(18.5336,6.7759)
(17.7189,6.6412)
(17.5153,6.7451)
(17.3116,6.8493)
(17.1079,6.9536)
(16.2933,6.8201)
(16.0896,6.9238)
(15.8859,7.0270)
(15.6823,7.1296)
(15.2749,7.2324)
(14.6640,7.3394)
(14.4603,7.4816)
(14.2566,7.5840)
(13.8493,7.6923)
(13.6456,7.9572)
(13.2383,8.0645)
(13.0346,8.1737)
(12.8310,8.2786)
(12.6273,8.3897)
(12.4236,8.5434)
(12.0163,8.4046)
(11.8126,8.2739)
(11.6090,8.4444)
(11.4053,8.6957)
(10.9980,8.5308)
(10.7943,8.6319)
(10.5906,9.1228)
(10.3870,9.5506)
(10.1833,9.3809)
(9.9796,9.4961)
(9.7760,9.7561)
(9.5723,9.6311)
(9.1650,9.4737)
(8.7576,9.2473)
(8.3503,8.9912)
(8.1466,9.1116)
(7.9430,9.3525)
(7.7393,9.1566)
(7.5356,8.9588)
(7.3320,9.8361)
(7.1283,9.5890)
(6.9246,9.4183)
(6.7210,9.9099)
(6.5173,9.6386)
(6.3136,9.8413)
(6.1100,10.0000)
(5.9063,10.1045)
(5.7026,10.4089)
(5.4990,10.0746)
(5.2953,9.7378)
(5.0916,10.6838)
(4.8880,10.8108)
(4.6843,10.4545)
(4.4807,10.1382)
(4.2770,10.2439)
(4.0733,9.8039)
(3.8697,9.4527)
(3.6660,9.0000)
(3.4623,8.5859)
(3.2587,8.2051)
(3.0550,7.9365)
(2.8513,7.5269)
(2.6477,7.0270)
(2.4440,6.5934)
(2.2403,6.1453)
(2.0367,5.6497)
(1.6293,5.1282)
(1.4257,4.7945)
(1.2220,4.3165)
(1.0183,3.7594)
(0.8147,3.4783)
(0.6110,5.2632)
(0.4073,3.5714)
(0.2037,2.6316)
(0.0000,0.0000)
(0.0,0.0000)};\addlegendentry{Our Model  (Synthetic + Real) (AP = 39.85)}
\addlegendentry{GNN (Synthetic + Real) (AP = 25.87)}
\addlegendentry{GNN (Only Synthetic) (AP = 5.35)}


==> figures/rp/real/argswap.tex <==
\addplot [draw=Peach, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.7046)
(98.7805,0.8046)
(94.3089,0.9046)
(89.0244,1.0046)
(85.3659,1.1047)
(82.1138,1.2047)
(77.6423,1.3048)
(74.3902,1.4049)
(69.5122,1.5049)
(69.1057,1.6255)
(66.2602,1.7256)
(64.2276,1.8257)
(59.7561,1.9258)
(55.6911,2.0260)
(52.8455,2.1263)
(49.5935,2.2263)
(45.1220,2.3266)
(44.7154,2.4592)
(40.2439,2.5595)
(39.8374,2.6602)
(37.8049,2.7605)
(32.5203,2.6552)
(30.8943,2.7556)
(28.4553,2.8560)
(28.0488,3.0572)
(27.6423,3.1584)
(26.0163,3.2587)
(25.6098,3.3600)
(23.9837,3.4604)
(23.5772,4.4241)
(23.1707,4.7619)
(21.9512,4.8649)
(21.5447,5.0669)
(20.7317,4.9515)
(19.9187,4.7665)
(19.5122,4.8682)
(19.1057,5.1762)
(18.6992,5.9202)
(18.2927,6.0241)
(17.4797,6.1254)
(17.0732,6.0086)
(16.2602,5.8394)
(15.8537,5.9724)
(15.4472,6.2500)
(14.6341,6.3604)
(14.2276,6.4695)
(13.8211,6.9672)
(13.4146,8.1281)
(12.6016,7.9082)
(12.1951,8.0214)
(11.7886,8.3095)
(11.3821,8.0692)
(10.9756,8.8525)
(10.5691,8.7248)
(10.1626,10.5485)
(9.7561,10.2128)
(9.3496,10.0437)
(8.9431,12.0879)
(8.5366,14.0940)
(8.1301,19.6078)
(7.7236,20.0000)
(7.3171,19.1489)
(6.9106,19.7674)
(6.5041,21.0526)
(6.0976,25.0000)
(5.6911,63.6364)
(5.2846,72.2222)
(4.8780,92.3077)
(4.4715,91.6667)
(4.0650,90.9091)
(3.6585,90.0000)
(3.2520,88.8889)
(2.8455,87.5000)
(2.4390,85.7143)
(2.0325,83.3333)
(1.6260,80.0000)
(1.2195,100.0000)
(0.0,100.0000)};
\addplot [draw=Plum, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.5687)
(99.1870,0.6687)
(97.5610,0.7687)
(93.9024,0.8687)
(88.2114,0.9688)
(81.7073,1.0688)
(76.8293,1.1688)
(72.7642,1.2688)
(69.9187,1.3689)
(66.2602,1.4690)
(58.9431,1.5691)
(49.1870,1.6692)
(46.7480,1.7692)
(38.2114,1.8695)
(36.1789,1.9699)
(30.8943,2.0703)
(30.4878,2.1708)
(29.2683,2.2713)
(28.8618,2.5558)
(26.0163,2.6567)
(25.6098,2.7571)
(25.2033,2.9356)
(23.9837,3.0365)
(23.5772,3.1368)
(23.1707,3.2386)
(22.7642,3.4230)
(22.3577,3.5234)
(20.7317,3.6247)
(20.3252,3.7965)
(19.9187,3.8982)
(19.5122,4.0000)
(18.2927,3.8793)
(17.4797,3.9815)
(17.0732,4.0816)
(16.6667,4.1837)
(15.4472,4.2841)
(15.0407,4.3891)
(14.6341,4.5627)
(14.2276,5.3929)
(13.8211,5.6013)
(13.4146,5.7093)
(13.0081,5.9590)
(12.6016,5.7944)
(12.1951,7.0423)
(11.7886,8.3095)
(11.3821,10.4089)
(10.9756,15.2542)
(10.5691,15.7576)
(10.1626,17.7305)
(9.7561,23.5294)
(9.3496,23.0000)
(8.9431,22.4490)
(8.5366,22.8261)
(8.1301,23.8095)
(7.7236,42.2222)
(7.3171,62.0690)
(6.9106,60.7143)
(6.5041,61.5385)
(6.0976,75.0000)
(5.6911,73.6842)
(5.2846,72.2222)
(4.8780,75.0000)
(4.4715,91.6667)
(4.0650,90.9091)
(3.6585,90.0000)
(3.2520,88.8889)
(2.8455,100.0000)
(0.0,100.0000)};
\addplot [draw=Cerulean, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.6502)
(98.3740,0.7502)
(89.8374,0.8503)
(79.2683,0.9503)
(71.1382,1.0503)
(66.6667,1.1503)
(58.5366,1.2503)
(39.4309,1.3504)
(27.2358,1.4505)
(26.8293,1.5508)
(26.4228,1.7464)
(26.0163,1.8599)
(25.6098,2.0019)
(23.1707,2.1025)
(22.7642,2.2030)
(22.3577,2.3595)
(21.9512,2.4873)
(21.5447,2.5879)
(21.1382,2.6887)
(20.7317,2.7899)
(20.3252,2.8902)
(19.5122,2.9907)
(18.2927,2.8883)
(17.8862,3.4510)
(17.4797,3.5923)
(17.0732,3.7267)
(16.6667,3.8936)
(16.2602,3.9960)
(15.8537,4.1096)
(15.4472,4.3133)
(15.0407,4.4153)
(14.6341,4.5169)
(14.2276,5.0072)
(13.4146,4.8889)
(13.0081,4.9922)
(12.6016,7.0295)
(12.1951,7.1429)
(11.7886,7.2500)
(11.3821,8.1395)
(10.9756,8.2569)
(10.5691,10.5691)
(10.1626,10.6838)
(9.7561,10.8108)
(9.3496,10.9524)
(8.9431,13.5802)
(8.5366,15.7895)
(8.1301,23.2558)
(7.7236,34.5455)
(7.3171,33.3333)
(6.9106,45.9459)
(6.5041,53.3333)
(6.0976,51.7241)
(5.6911,50.0000)
(5.2846,61.9048)
(4.8780,85.7143)
(4.4715,84.6154)
(4.0650,83.3333)
(3.6585,100.0000)
(0.0,100.0000)};

\addlegendentry{Our Full Method (AP = 8.49)}
\addlegendentry{Mix (AP = 9.33)}
\addlegendentry{Only Synthetic (AP = 8.31)}

==> figures/rp/real/var-misuse.tex <==
\addplot [draw=Peach, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.9871)
(99.1071,1.0871)
(98.5119,1.1871)
(97.0238,1.2872)
(96.4286,1.3872)
(95.8333,1.4872)
(94.3452,1.5873)
(93.4524,1.6874)
(92.8571,1.7875)
(92.2619,1.8875)
(91.3690,1.9876)
(91.0714,2.0876)
(90.7738,2.2206)
(88.9881,2.3207)
(87.5000,2.4207)
(86.6071,2.5208)
(85.1190,2.6212)
(83.6310,2.7213)
(83.3333,2.8214)
(83.0357,2.9215)
(81.2500,3.0216)
(80.9524,3.1218)
(80.6548,3.2220)
(79.1667,3.3221)
(77.9762,3.4222)
(77.3810,3.5230)
(77.0833,3.6234)
(76.7857,3.7235)
(76.1905,3.8237)
(74.4048,3.9240)
(74.1071,4.0246)
(73.5119,4.1249)
(72.9167,4.2256)
(72.6190,4.3262)
(71.4286,4.4264)
(70.8333,4.5264)
(70.2381,4.6275)
(69.0476,4.7279)
(68.7500,4.8316)
(66.6667,4.9317)
(66.3690,5.0327)
(65.7738,5.1336)
(65.4762,5.2344)
(65.1786,5.3808)
(64.5833,5.4812)
(64.2857,5.6265)
(63.3929,5.7273)
(63.0952,5.8274)
(62.7976,5.9605)
(61.9048,6.0606)
(61.6071,6.1607)
(60.1190,6.2616)
(59.2262,6.3619)
(58.9286,6.4621)
(58.6310,6.6130)
(57.4405,6.7130)
(57.1429,6.8133)
(55.9524,6.9143)
(54.7619,7.0149)
(54.1667,7.1149)
(53.5714,7.2173)
(53.2738,7.3181)
(52.9762,7.4947)
(52.6786,7.5966)
(52.3810,7.6990)
(52.0833,7.8021)
(51.7857,8.0184)
(51.4881,8.1221)
(49.1071,8.2253)
(47.9167,8.3290)
(47.6190,8.4971)
(47.3214,8.5992)
(47.0238,9.0909)
(46.7262,9.1920)
(46.4286,9.5588)
(46.1310,9.6633)
(45.8333,9.7654)
(45.2381,9.8701)
(44.6429,9.9734)
(44.3452,10.1017)
(44.0476,10.2069)
(43.1548,10.3129)
(42.8571,10.4197)
(42.5595,10.5769)
(41.9643,10.4755)
(41.3690,10.5784)
(40.7738,10.6864)
(40.4762,10.7937)
(39.8810,10.8943)
(39.2857,11.0000)
(38.6905,11.1016)
(37.5000,11.2100)
(37.2024,11.3740)
(36.9048,11.4815)
(36.6071,11.5819)
(36.0119,11.4801)
(35.7143,11.6732)
(35.4167,11.7822)
(35.1190,12.0041)
(34.8214,12.2642)
(34.5238,12.5405)
(34.2262,12.6513)
(33.9286,12.7517)
(32.7381,12.8655)
(32.4405,13.0539)
(32.1429,14.5749)
(31.8452,14.6776)
(31.2500,14.5028)
(30.6548,14.6099)
(30.3571,14.7186)
(30.0595,15.1880)
(29.7619,15.3374)
(29.4643,15.4446)
(29.1667,16.3606)
(28.8690,16.6381)
(28.5714,16.8717)
(27.9762,16.7260)
(27.6786,16.6071)
(27.3810,16.7273)
(27.0833,16.8519)
(26.7857,17.7515)
(26.4881,18.1633)
(26.1905,20.1373)
(25.8929,21.3759)
(25.5952,21.1823)
(25.2976,22.7273)
(25.0000,22.5201)
(24.7024,23.6467)
(24.4048,24.9240)
(24.1071,25.5521)
(23.8095,25.9740)
(23.5119,26.8707)
(23.2143,26.7123)
(22.9167,26.5517)
(22.6190,27.9412)
(22.3214,29.6443)
(22.0238,29.4821)
(21.7262,29.9180)
(21.4286,30.1255)
(21.1310,29.9578)
(20.8333,29.7872)
(20.5357,30.0000)
(20.2381,32.5359)
(19.9405,34.5361)
(19.6429,34.3750)
(19.3452,34.0314)
(19.0476,34.9727)
(18.7500,41.4474)
(18.4524,42.4658)
(18.1548,46.2121)
(17.8571,46.5116)
(17.5595,46.0938)
(17.2619,46.7742)
(16.9643,46.3415)
(16.6667,46.6667)
(16.3690,47.0085)
(16.0714,47.3684)
(15.4762,46.8468)
(15.1786,47.2222)
(14.8810,48.5437)
(14.5833,49.4949)
(14.2857,50.0000)
(13.9881,57.3171)
(13.6905,56.7901)
(13.3929,64.2857)
(13.0952,65.6716)
(12.7976,65.1515)
(12.5000,64.6154)
(12.2024,64.0625)
(11.9048,66.6667)
(11.6071,66.1017)
(11.3095,65.5172)
(11.0119,66.0714)
(10.7143,65.4545)
(10.4167,64.8148)
(10.1190,65.3846)
(9.8214,67.3469)
(9.5238,68.0851)
(9.2262,68.8889)
(8.9286,68.1818)
(8.6310,67.4419)
(8.3333,71.7949)
(8.0357,77.1429)
(7.7381,78.7879)
(7.4405,86.2069)
(7.1429,85.7143)
(6.8452,88.4615)
(6.5476,88.0000)
(6.2500,91.3043)
(5.9524,95.2381)
(5.6548,95.0000)
(5.3571,94.7368)
(5.0595,94.4444)
(4.7619,94.1176)
(4.4643,93.7500)
(4.1667,93.3333)
(3.8690,92.8571)
(3.5714,92.3077)
(3.2738,91.6667)
(2.9762,90.9091)
(2.6786,90.0000)
(2.3810,100.0000)
(0.0,100.0000)};
\addplot [draw=Plum, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.7321)
(99.7024,0.8321)
(98.5119,0.9321)
(98.2143,1.0824)
(97.0238,1.1824)
(95.5357,1.2824)
(94.6429,1.3824)
(92.8571,1.4825)
(91.0714,1.5825)
(88.6905,1.6826)
(87.5000,1.7826)
(84.8214,1.8827)
(81.8452,1.9827)
(80.3571,2.0829)
(76.1905,2.1830)
(72.3214,2.2832)
(70.8333,2.3833)
(70.2381,2.4834)
(66.6667,2.5836)
(63.3929,2.6836)
(60.4167,2.7839)
(58.3333,2.8840)
(53.5714,2.9841)
(52.6786,3.0842)
(50.2976,3.1845)
(50.0000,3.2851)
(44.9405,3.3857)
(44.0476,3.4865)
(43.7500,3.5994)
(42.5595,3.6999)
(36.9048,3.8002)
(36.6071,3.9010)
(34.5238,4.0014)
(33.6310,4.1016)
(33.0357,4.2030)
(32.4405,4.3032)
(32.1429,4.4944)
(31.2500,4.5952)
(28.5714,4.6967)
(28.2738,4.7980)
(27.6786,4.8999)
(27.3810,5.2874)
(27.0833,5.3878)
(26.7857,5.6782)
(25.0000,5.5777)
(24.1071,5.6802)
(23.8095,5.7803)
(23.5119,5.8824)
(23.2143,5.9862)
(22.9167,6.0870)
(22.6190,6.1889)
(22.0238,6.2925)
(21.7262,6.4035)
(21.4286,6.5634)
(21.1310,6.8269)
(20.5357,6.7121)
(20.2381,6.8136)
(19.6429,6.6332)
(19.0476,6.7368)
(18.7500,7.0078)
(18.4524,7.8580)
(18.1548,8.0052)
(17.5595,8.1155)
(17.2619,8.0000)
(16.6667,7.8984)
(16.3690,7.7793)
(15.4762,7.8907)
(15.1786,8.1994)
(14.8810,9.2764)
(14.5833,10.2941)
(14.2857,10.5033)
(13.9881,10.6095)
(13.6905,11.5578)
(13.3929,12.0643)
(13.0952,11.8598)
(12.7976,11.7486)
(12.5000,13.7255)
(12.2024,13.5314)
(11.9048,16.5289)
(11.6071,17.0306)
(11.3095,17.5926)
(11.0119,18.5930)
(10.7143,18.8482)
(10.4167,19.2308)
(10.1190,19.7674)
(9.8214,19.6429)
(9.5238,20.7792)
(9.2262,20.6667)
(8.9286,21.4286)
(8.6310,21.8045)
(8.3333,22.0472)
(8.0357,21.4286)
(7.7381,21.6667)
(7.4405,21.9298)
(7.1429,21.2389)
(6.8452,24.7312)
(6.5476,25.2874)
(6.2500,29.1667)
(5.9524,28.1690)
(5.6548,28.3582)
(5.3571,27.2727)
(5.0595,31.4815)
(4.7619,31.3725)
(4.4643,34.0909)
(4.1667,40.0000)
(3.8690,39.3939)
(3.5714,37.5000)
(3.2738,36.6667)
(2.9762,40.0000)
(2.6786,37.5000)
(2.3810,34.7826)
(2.0833,38.8889)
(1.7857,35.2941)
(1.4881,38.4615)
(1.1905,36.3636)
(0.8929,75.0000)
(0.5952,66.6667)
(0.2976,50.0000)
(0.0000,100.0000)
(0.0,100.0000)};
\addplot [draw=Cerulean, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,0.8281)
(98.8095,0.9281)
(98.5119,1.0784)
(96.7262,1.1784)
(94.3452,1.2784)
(92.2619,1.3785)
(90.1786,1.4785)
(86.6071,1.5785)
(84.2262,1.6785)
(81.2500,1.7786)
(79.1667,1.8787)
(73.5119,1.9787)
(65.7738,2.0788)
(64.2857,2.1790)
(61.9048,2.2792)
(61.6071,2.3793)
(60.7143,2.4793)
(60.1190,2.5795)
(52.3810,2.6797)
(51.1905,2.7800)
(49.1071,2.8801)
(46.4286,2.9805)
(44.0476,3.0808)
(37.7976,3.1814)
(36.9048,3.2822)
(35.4167,3.3826)
(35.1190,3.4829)
(33.9286,3.5838)
(31.5476,3.6844)
(31.2500,3.7851)
(30.6548,3.8853)
(28.8690,3.9868)
(28.2738,4.0878)
(27.6786,4.1892)
(25.0000,4.2901)
(24.1071,4.3902)
(23.8095,4.4919)
(23.5119,4.5930)
(23.2143,4.6931)
(22.9167,4.9518)
(22.3214,5.0539)
(22.0238,5.1568)
(20.5357,5.2591)
(19.3452,5.1587)
(19.0476,5.2588)
(18.4524,5.1197)
(18.1548,5.2226)
(17.5595,5.3249)
(17.2619,5.4256)
(16.9643,5.5286)
(16.6667,5.6338)
(16.3690,5.8263)
(15.7738,5.6503)
(15.4762,5.7522)
(15.1786,5.8553)
(14.8810,6.0096)
(14.5833,6.1097)
(14.2857,6.2176)
(13.9881,6.3257)
(13.6905,7.3132)
(13.3929,8.0501)
(12.7976,7.9482)
(12.2024,8.0550)
(11.9048,8.2988)
(11.6071,9.2417)
(11.3095,9.0909)
(10.7143,8.9552)
(10.4167,9.3085)
(10.1190,10.7256)
(9.8214,11.0738)
(9.5238,11.2676)
(9.2262,12.6016)
(8.9286,12.2449)
(8.6310,12.0332)
(8.3333,13.9303)
(8.0357,13.7755)
(7.7381,13.9037)
(7.4405,14.0449)
(7.1429,14.2012)
(6.8452,14.0244)
(6.5476,15.6028)
(6.2500,15.7895)
(5.9524,15.1515)
(5.6548,15.3226)
(5.3571,15.1261)
(5.0595,14.4068)
(4.7619,14.2857)
(4.4643,14.4231)
(4.1667,15.5556)
(3.8690,18.3099)
(3.5714,28.5714)
(3.2738,34.3750)
(2.9762,33.3333)
(2.6786,34.6154)
(2.3810,33.3333)
(2.0833,36.8421)
(1.7857,40.0000)
(1.4881,45.4545)
(1.1905,40.0000)
(0.8929,33.3333)
(0.5952,40.0000)
(0.2976,25.0000)
(0.0000,0.0000)
(0.0,0.0000)};

\addlegendentry{Our Full Method (AP = 20.96)}
\addlegendentry{Mix (AP = 7.27)}
\addlegendentry{Only Synthetic (AP = 5.24)}

==> figures/rp/real/wrong-bin-op.tex <==
\addplot [draw=Peach, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,1.8454)
(99.5927,1.9454)
(99.3890,2.3306)
(98.9817,2.4306)
(98.3707,2.5307)
(97.7597,2.6307)
(97.5560,2.7637)
(97.3523,2.8638)
(97.1487,2.9640)
(96.5377,3.0642)
(96.3340,3.1643)
(96.1303,3.2644)
(95.9267,3.3645)
(95.7230,3.4645)
(95.3157,3.5646)
(95.1120,3.6648)
(94.9084,3.7650)
(94.5010,3.8651)
(94.2974,3.9651)
(93.6864,4.0654)
(93.4827,4.2690)
(93.0754,4.3690)
(92.8717,4.5041)
(92.4644,4.6045)
(92.2607,4.7330)
(91.6497,4.8335)
(91.0387,4.9338)
(90.8350,5.1602)
(90.6314,5.2607)
(90.4277,5.3610)
(90.2240,5.4610)
(89.8167,5.5612)
(89.6130,5.8737)
(89.4094,6.0938)
(89.2057,6.2022)
(88.5947,6.3025)
(88.3910,6.4031)
(87.9837,6.5031)
(87.1690,6.6039)
(86.9654,6.7043)
(86.7617,6.8062)
(86.5580,6.9072)
(86.3544,7.0083)
(86.1507,7.1092)
(85.7434,7.2101)
(85.5397,7.5080)
(85.3360,7.6460)
(84.9287,7.7466)
(84.7251,7.9163)
(84.3177,8.0170)
(84.1141,8.1171)
(83.9104,8.2186)
(83.7067,8.4900)
(83.5031,8.9053)
(83.2994,9.1478)
(83.0957,9.3685)
(82.8921,9.4695)
(82.6884,9.9632)
(82.4847,10.0646)
(82.2811,10.6288)
(82.0774,10.8333)
(81.8737,10.9656)
(80.2444,11.0674)
(80.0407,11.1679)
(79.8371,11.2871)
(79.6334,11.4461)
(79.4297,11.5556)
(78.8187,11.6566)
(78.6151,11.7575)
(78.4114,11.8608)
(78.2077,12.2021)
(77.3931,12.3057)
(77.1894,12.4059)
(76.9857,12.5083)
(76.7821,12.7797)
(76.3747,12.8822)
(76.1711,12.9861)
(75.9674,13.0969)
(75.7637,13.2009)
(75.5601,13.3935)
(75.3564,13.4938)
(75.1527,13.7635)
(74.3381,13.8678)
(74.1344,14.1524)
(73.9308,14.2577)
(73.7271,14.5090)
(73.5234,14.6569)
(73.3198,14.7601)
(73.1161,15.3419)
(72.7088,15.4479)
(72.5051,15.5526)
(72.3014,15.7358)
(72.0978,15.8531)
(71.8941,15.9584)
(71.6904,16.0951)
(71.4868,16.3104)
(71.2831,16.4706)
(71.0794,16.6032)
(70.8758,16.8197)
(70.6721,17.0265)
(70.4684,17.3173)
(70.2648,17.4242)
(70.0611,17.5331)
(69.8574,17.9769)
(69.6538,18.4566)
(69.4501,18.8086)
(69.2464,19.0157)
(69.0428,19.6979)
(68.8391,20.3737)
(68.6354,20.7640)
(68.4318,20.9738)
(68.2281,21.1356)
(68.0244,21.3010)
(67.8208,22.0093)
(67.6171,22.1629)
(67.4134,23.1631)
(67.2098,23.4209)
(67.0061,23.5336)
(66.8024,24.3685)
(66.5988,24.5495)
(66.3951,25.4887)
(66.1914,25.6917)
(65.9878,26.0450)
(65.7841,26.3458)
(65.5804,26.4585)
(65.3768,27.5064)
(65.1731,27.6339)
(64.9695,27.7391)
(64.7658,27.9683)
(64.5621,28.2028)
(64.1548,28.0999)
(63.9511,28.3906)
(63.7475,28.5064)
(63.5438,28.9157)
(63.3401,30.2824)
(63.1365,30.4519)
(62.9328,30.5638)
(62.7291,30.7692)
(62.5255,31.1992)
(62.3218,31.3846)
(61.9145,31.5026)
(61.7108,32.3028)
(61.5071,32.4034)
(61.3035,32.9322)
(61.0998,33.0396)
(60.8961,33.2592)
(60.6925,33.3707)
(60.4888,33.7117)
(60.2851,33.9839)
(60.0815,34.7059)
(59.8778,34.8754)
(59.6741,35.0060)
(59.4705,35.1384)
(59.2668,35.2727)
(59.0631,36.7089)
(58.8595,37.0988)
(58.6558,37.2574)
(58.4521,37.3698)
(58.2485,37.4836)
(58.0448,38.5656)
(57.8411,39.0110)
(57.6375,39.3056)
(57.4338,40.2282)
(57.2301,40.7837)
(57.0265,41.1160)
(56.4155,41.2202)
(56.2118,41.3793)
(56.0081,41.5408)
(55.8045,41.8321)
(55.6008,42.1296)
(55.3971,42.2360)
(55.1935,42.3438)
(54.9898,42.6540)
(54.3788,42.5159)
(54.1752,42.8341)
(53.9715,43.3715)
(53.7678,43.4926)
(53.5642,43.7604)
(53.1568,43.8655)
(52.5458,43.7288)
(52.3422,44.9301)
(52.1385,46.4610)
(51.7312,46.3504)
(51.5275,46.6790)
(51.3238,46.9274)
(51.1202,47.0919)
(50.7128,46.9811)
(50.5092,47.2381)
(50.3055,47.1374)
(49.8982,47.2973)
(49.6945,47.1954)
(49.4908,47.0930)
(49.2872,47.7318)
(48.8798,47.9042)
(48.6762,48.0885)
(48.4725,47.9839)
(48.2688,48.1707)
(48.0652,48.3607)
(47.8615,48.2546)
(47.6578,48.1481)
(47.4542,48.3402)
(47.2505,49.5726)
(47.0468,49.6774)
(46.8432,49.8915)
(46.6395,50.0000)
(46.4358,50.1099)
(46.0285,50.0000)
(45.8248,49.8891)
(45.6212,50.0000)
(45.4175,50.9132)
(45.2138,51.1521)
(45.0102,51.2761)
(44.8065,51.4019)
(44.6029,51.5294)
(44.3992,51.6588)
(44.1955,51.5439)
(43.9919,52.3002)
(43.7882,52.4390)
(43.5845,52.5799)
(43.3809,52.7228)
(43.1772,52.6055)
(42.9735,53.0151)
(42.7699,53.2995)
(42.5662,53.1807)
(42.1589,53.0769)
(41.9552,53.2300)
(41.7515,53.3854)
(41.5479,53.2637)
(41.3442,53.1414)
(41.1405,53.2982)
(40.9369,53.7433)
(40.7332,54.3478)
(40.5295,54.5205)
(40.1222,54.4199)
(39.9185,54.5961)
(39.7149,54.4693)
(39.3075,54.3662)
(39.1039,54.2373)
(38.9002,54.8851)
(38.6965,54.7550)
(38.4929,54.9419)
(38.2892,54.8105)
(38.0855,54.6784)
(37.8819,54.5455)
(37.6782,54.7337)
(37.4745,54.9254)
(37.2709,55.1205)
(37.0672,56.8750)
(36.8635,57.0978)
(36.6599,57.3248)
(35.8452,57.1429)
(35.6415,57.5658)
(35.2342,57.6667)
(35.0305,57.9125)
(34.8269,57.7703)
(34.6232,58.0205)
(34.4196,57.8767)
(34.2159,58.9474)
(34.0122,58.8028)
(33.8086,58.6572)
(33.6049,58.9286)
(33.4012,59.2058)
(33.1976,59.0580)
(32.9939,59.3407)
(32.7902,59.1912)
(32.5866,59.0406)
(32.1792,59.1760)
(31.9756,59.4697)
(31.7719,59.3156)
(31.5682,60.3113)
(31.3646,60.6299)
(31.1609,60.4743)
(30.9572,60.8000)
(30.7536,60.6426)
(30.5499,60.9756)
(30.3462,61.5702)
(30.1426,61.4108)
(29.9389,61.7647)
(29.7352,62.1277)
(29.5316,61.9658)
(29.3279,62.0690)
(29.1242,62.1739)
(28.9206,62.0087)
(28.7169,61.8421)
(28.5132,62.2222)
(28.3096,62.3318)
(28.1059,62.1622)
(27.9022,61.9910)
(27.6986,61.8182)
(27.4949,61.6438)
(27.2912,61.7512)
(27.0876,61.8605)
(26.8839,61.6822)
(26.6802,61.5023)
(26.4766,61.9048)
(26.2729,61.7225)
(26.0692,62.4390)
(25.8656,62.8713)
(25.6619,63.0000)
(25.4582,62.8141)
(25.2546,62.9442)
(25.0509,62.7551)
(24.8473,62.8866)
(24.6436,64.3617)
(24.4399,64.5161)
(24.2363,65.7459)
(24.0326,65.9218)
(23.8289,65.7303)
(23.6253,65.9091)
(23.4216,65.7143)
(23.2179,66.2791)
(23.0143,67.6647)
(22.8106,67.4699)
(22.6069,67.6829)
(22.4033,67.9012)
(22.1996,68.5535)
(21.9959,68.7898)
(21.7923,68.5897)
(21.5886,68.3871)
(21.3849,68.1818)
(21.1813,68.4211)
(20.9776,69.1275)
(20.7739,68.9189)
(20.5703,69.1781)
(20.3666,68.9655)
(20.1629,68.7500)
(19.9593,69.0141)
(19.7556,68.7943)
(19.5519,70.5882)
(19.3483,70.8955)
(19.1446,71.2121)
(18.9409,70.9924)
(18.7373,70.7692)
(18.5336,70.5426)
(18.3299,70.3125)
(18.1263,70.0787)
(17.9226,69.8413)
(17.7189,69.6000)
(17.5153,69.9187)
(17.3116,69.6721)
(17.1079,69.4215)
(16.9043,69.1667)
(16.7006,68.9076)
(16.4969,68.6441)
(16.2933,68.3761)
(16.0896,68.1034)
(15.8859,67.8261)
(15.6823,67.5439)
(15.4786,68.4685)
(15.2749,68.1818)
(15.0713,68.5185)
(14.8676,68.2243)
(14.6640,67.9245)
(14.4603,67.6190)
(14.2566,67.3077)
(14.0530,67.6471)
(13.8493,67.3267)
(13.6456,67.0000)
(13.4420,66.6667)
(13.2383,66.3265)
(13.0346,66.6667)
(12.8310,66.3158)
(12.6273,65.9574)
(12.4236,65.5914)
(12.2200,65.2174)
(12.0163,65.5556)
(11.8126,65.1685)
(11.6090,64.7727)
(11.4053,65.1163)
(11.2016,64.7059)
(10.9980,64.2857)
(10.7943,63.8554)
(10.5906,63.4146)
(10.3870,64.5570)
(10.1833,64.1026)
(9.9796,63.6364)
(9.7760,63.1579)
(9.5723,62.6667)
(9.3686,62.1622)
(9.1650,61.6438)
(8.9613,61.1111)
(8.7576,61.4286)
(8.5540,60.8696)
(8.3503,60.2941)
(8.1466,59.7015)
(7.9430,60.9375)
(7.7393,60.3175)
(7.5356,59.6774)
(7.3320,59.0164)
(7.1283,59.3220)
(6.9246,58.6207)
(6.7210,57.8947)
(6.5173,60.3774)
(6.3136,59.6154)
(6.1100,58.8235)
(5.9063,58.0000)
(5.7026,57.1429)
(5.4990,56.2500)
(5.2953,55.3191)
(5.0916,59.5238)
(4.8880,58.5366)
(4.6843,57.5000)
(4.4807,57.8947)
(4.2770,56.7568)
(4.0733,58.8235)
(3.8697,57.5758)
(3.6660,58.0645)
(3.4623,56.6667)
(3.2587,59.2593)
(3.0550,60.0000)
(2.8513,58.3333)
(2.6477,56.5217)
(2.4440,60.0000)
(2.2403,57.8947)
(2.0367,55.5556)
(1.8330,52.9412)
(1.6293,57.1429)
(1.4257,53.8462)
(1.2220,60.0000)
(1.0183,55.5556)
(0.8147,50.0000)
(0.6110,60.0000)
(0.4073,66.6667)
(0.2037,50.0000)
(0.0000,100.0000)
(0.0,100.0000)};
\addplot [draw=Plum, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,1.4679)
(99.7963,1.5679)
(99.5927,1.6949)
(99.1853,1.7949)
(98.9817,1.9156)
(98.1670,2.0156)
(97.9633,2.1157)
(97.7597,2.2158)
(97.5560,2.4004)
(96.9450,2.5005)
(96.3340,2.6006)
(95.1120,2.7007)
(94.0937,2.8007)
(93.6864,2.9007)
(93.0754,3.0009)
(92.4644,3.1009)
(91.0387,3.2011)
(90.2240,3.3013)
(89.8167,3.4015)
(89.2057,3.5015)
(88.7984,3.6015)
(88.3910,3.7018)
(86.5580,3.8021)
(86.1507,3.9022)
(85.9470,4.0133)
(85.5397,4.1136)
(84.1141,4.2139)
(82.6884,4.3141)
(81.8737,4.4142)
(80.0407,4.5146)
(79.6334,4.6147)
(78.8187,4.7149)
(76.9857,4.8153)
(74.1344,4.9156)
(73.5234,5.0160)
(72.5051,5.1164)
(71.4868,5.2170)
(70.8758,5.3170)
(70.0611,5.4173)
(69.8574,5.5180)
(68.6354,5.6185)
(68.2281,5.7187)
(68.0244,5.8188)
(67.2098,5.9193)
(67.0061,6.0201)
(65.9878,6.1201)
(65.5804,6.2210)
(65.1731,6.3216)
(64.9695,6.4224)
(63.3401,6.5227)
(62.9328,6.6238)
(62.7291,6.7249)
(62.3218,6.8258)
(61.9145,6.9264)
(61.5071,7.0265)
(60.2851,7.1274)
(59.2668,7.2280)
(59.0631,7.3288)
(58.0448,7.4296)
(57.8411,7.5312)
(57.0265,7.6315)
(56.2118,7.7333)
(55.3971,7.8341)
(55.1935,7.9356)
(54.9898,8.0357)
(54.1752,8.1370)
(53.5642,8.2393)
(53.3605,8.8156)
(52.9532,8.9163)
(52.5458,9.0178)
(52.1385,9.1201)
(51.3238,9.2206)
(51.1202,9.4361)
(50.9165,9.5822)
(50.7128,9.6849)
(50.1018,9.7852)
(49.8982,10.1365)
(49.6945,10.2392)
(49.4908,10.3404)
(48.8798,10.4439)
(48.2688,10.5474)
(47.4542,10.6490)
(47.0468,10.7492)
(46.8432,10.9005)
(46.6395,11.0043)
(46.4358,11.1710)
(46.2322,11.2711)
(46.0285,11.3739)
(45.8248,11.5266)
(45.6212,11.6303)
(45.2138,11.7336)
(45.0102,11.9978)
(44.8065,12.1012)
(44.6029,12.2074)
(44.1955,12.3086)
(43.1772,12.4122)
(42.9735,12.6955)
(42.3625,12.5908)
(42.1589,12.6916)
(41.7515,12.7965)
(41.5479,12.9032)
(41.3442,13.0045)
(39.1039,12.8946)
(38.9002,13.0020)
(38.2892,12.8855)
(37.2709,12.7704)
(36.8635,12.6662)
(36.6599,12.7750)
(36.4562,12.8777)
(35.8452,12.7260)
(35.6415,12.8299)
(35.0305,12.6657)
(34.6232,12.7724)
(34.0122,12.8759)
(33.4012,12.9850)
(32.9939,12.8571)
(32.7902,13.0576)
(32.3829,12.9268)
(31.7719,13.0326)
(31.5682,13.1356)
(31.3646,13.2416)
(30.9572,13.1374)
(30.7536,13.2456)
(30.1426,13.1439)
(29.9389,13.3394)
(29.7352,13.4562)
(29.5316,13.5641)
(28.5132,13.4615)
(28.1059,13.3205)
(27.4949,13.1965)
(26.6802,13.2995)
(26.4766,13.4021)
(26.0692,13.5021)
(25.6619,13.3475)
(25.4582,13.8274)
(25.2546,13.9326)
(25.0509,14.0411)
(24.6436,13.8603)
(24.4399,13.9697)
(24.2363,14.2686)
(24.0326,14.1657)
(23.8289,14.2683)
(23.4216,14.1278)
(23.0143,14.2317)
(22.6069,14.0863)
(22.4033,14.1935)
(22.1996,14.3421)
(21.5886,14.2282)
(21.3849,14.3443)
(21.1813,15.0725)
(20.9776,15.2367)
(20.7739,15.4312)
(20.5703,15.5385)
(20.3666,15.4083)
(20.1629,15.5172)
(19.9593,15.6300)
(19.7556,15.7468)
(19.5519,15.6352)
(19.3483,15.9933)
(19.1446,15.8784)
(18.9409,16.0622)
(18.7373,16.1687)
(18.5336,16.2791)
(18.3299,16.5138)
(18.1263,16.6355)
(17.9226,16.7619)
(17.7189,16.6031)
(17.5153,16.7315)
(17.3116,16.9323)
(17.1079,17.2485)
(16.9043,17.3640)
(16.7006,17.2632)
(16.4969,17.3820)
(16.2933,17.2786)
(16.0896,17.4009)
(15.8859,17.5281)
(15.6823,17.7011)
(15.4786,17.5115)
(15.2749,17.3611)
(15.0713,17.4941)
(14.8676,17.6329)
(14.6640,18.0905)
(14.4603,18.2051)
(14.2566,18.3727)
(14.0530,19.1667)
(13.8493,20.9231)
(13.6456,21.0692)
(13.2383,20.8333)
(13.0346,21.0526)
(12.8310,20.8609)
(12.6273,20.7358)
(12.4236,20.8904)
(12.2200,20.6897)
(12.0163,20.8481)
(11.8126,21.5613)
(11.6090,21.7557)
(11.4053,21.4559)
(11.2016,21.8254)
(10.9980,21.6867)
(10.7943,21.8107)
(10.5906,21.9409)
(10.3870,22.0779)
(10.1833,22.7273)
(9.9796,23.2227)
(9.7760,23.4146)
(9.5723,23.0392)
(9.3686,23.2323)
(9.1650,22.8426)
(8.9613,23.1579)
(8.7576,24.4318)
(8.5540,24.5614)
(8.3503,24.8485)
(8.1466,24.5399)
(7.9430,24.2236)
(7.7393,24.0506)
(7.5356,24.6667)
(7.3320,24.4898)
(7.1283,24.3056)
(6.9246,23.9437)
(6.5173,23.3577)
(6.3136,22.9630)
(6.1100,22.7273)
(5.9063,22.1374)
(5.7026,23.5294)
(5.4990,24.7706)
(5.2953,26.5306)
(5.0916,26.3158)
(4.8880,26.0870)
(4.6843,25.2747)
(4.4807,24.4444)
(4.2770,24.1379)
(4.0733,23.5294)
(3.8697,25.6757)
(3.6660,27.2727)
(3.4623,26.5625)
(3.2587,27.5862)
(3.0550,28.8462)
(2.8513,28.5714)
(2.6477,27.6596)
(2.4440,26.0870)
(2.2403,28.2051)
(2.0367,27.0270)
(1.8330,28.1250)
(1.6293,26.6667)
(1.4257,24.1379)
(1.2220,23.0769)
(1.0183,25.0000)
(0.6110,20.0000)
(0.4073,16.6667)
(0.2037,12.5000)
(0.0000,100.0000)
(0.0,100.0000)};
\addplot [draw=Cerulean, line width=0.7pt, const plot mark left] 
 coordinates { %
(100.0000,1.4627)
(99.7963,1.5627)
(99.3890,1.6627)
(99.1853,1.8916)
(98.9817,2.0074)
(98.7780,2.1075)
(98.3707,2.2077)
(98.1670,2.3078)
(97.5560,2.4079)
(96.9450,2.5079)
(96.7413,2.6080)
(96.5377,2.7081)
(96.3340,2.8081)
(96.1303,2.9082)
(95.3157,3.0083)
(94.7047,3.1085)
(94.2974,3.2086)
(93.6864,3.3086)
(93.2790,3.4088)
(92.8717,3.5088)
(91.2424,3.6088)
(90.2240,3.7090)
(90.0204,3.8090)
(89.8167,3.9092)
(88.3910,4.0092)
(88.1874,4.1093)
(87.5764,4.2095)
(87.3727,4.3098)
(85.9470,4.4101)
(84.5214,4.5104)
(83.0957,4.6107)
(81.6701,4.7110)
(80.8554,4.8115)
(79.4297,4.9118)
(78.0041,5.0124)
(75.5601,5.1130)
(73.7271,5.2131)
(72.0978,5.3137)
(71.4868,5.4142)
(68.8391,5.5148)
(67.6171,5.6157)
(65.9878,5.7163)
(64.7658,5.8167)
(63.5438,5.9169)
(62.1181,6.0170)
(61.5071,6.1171)
(61.3035,6.2177)
(60.0815,6.3183)
(59.4705,6.4190)
(59.2668,6.5778)
(59.0631,6.6789)
(58.8595,6.7793)
(58.0448,6.8807)
(57.8411,6.9813)
(57.6375,7.0856)
(57.0265,7.1869)
(56.8228,7.2884)
(55.3971,7.3893)
(54.1752,7.4908)
(53.9715,7.6501)
(53.7678,7.7761)
(53.5642,8.0037)
(53.3605,8.1039)
(52.5458,8.2061)
(52.1385,8.3063)
(51.9348,8.4075)
(51.7312,8.5092)
(51.5275,8.7151)
(51.3238,9.0975)
(51.1202,9.2313)
(50.9165,9.3318)
(50.7128,9.4354)
(49.8982,9.5368)
(49.6945,9.6405)
(48.8798,9.7442)
(48.4725,9.8469)
(48.0652,9.9494)
(47.6578,10.0515)
(47.4542,10.1525)
(46.8432,10.2541)
(46.6395,10.5774)
(46.4358,10.6792)
(46.2322,10.9821)
(46.0285,11.0839)
(45.8248,11.1885)
(45.6212,11.2960)
(45.4175,11.4008)
(45.2138,11.5385)
(45.0102,11.6438)
(44.8065,11.7459)
(43.7882,11.8523)
(43.5845,11.9553)
(43.3809,12.0612)
(42.7699,12.1669)
(41.7515,12.0305)
(41.5479,12.1356)
(41.3442,12.2363)
(41.1405,12.3396)
(40.9369,12.4845)
(40.5295,12.5870)
(40.3259,12.6923)
(39.7149,12.7953)
(38.6965,12.8988)
(38.4929,13.0705)
(36.0489,12.9481)
(35.4379,12.8130)
(35.2342,12.9201)
(34.8269,12.7994)
(34.4196,12.6972)
(33.8086,12.5758)
(33.4012,12.4525)
(32.7902,12.3466)
(32.3829,12.2214)
(31.7719,12.1118)
(31.1609,11.9812)
(30.7536,11.8617)
(30.3462,11.7231)
(29.7352,11.5873)
(29.3279,11.4741)
(28.7169,11.3253)
(28.1059,11.2104)
(27.6986,11.0749)
(27.0876,10.9465)
(25.8656,10.8085)
(25.4582,10.7021)
(25.0509,10.5579)
(23.8289,10.4278)
(23.0143,10.5312)
(22.8106,10.6363)
(22.1996,10.5010)
(21.3849,10.3960)
(21.1813,10.5799)
(20.7739,10.4615)
(20.5703,10.5649)
(19.9593,10.4478)
(19.1446,10.2957)
(18.7373,10.4072)
(18.5336,10.5446)
(18.3299,10.6509)
(17.7189,10.5455)
(17.5153,10.6568)
(17.3116,10.7595)
(16.9043,10.5867)
(16.7006,10.9188)
(16.4969,11.0204)
(16.2933,11.1266)
(16.0896,11.8087)
(15.8859,12.5806)
(15.6823,13.1175)
(15.4786,13.2404)
(15.2749,13.4650)
(15.0713,13.6280)
(14.8676,13.7476)
(14.6640,14.1454)
(14.2566,13.9721)
(14.0530,14.0816)
(13.8493,14.2857)
(13.6456,14.4086)
(13.2383,14.2857)
(13.0346,15.3846)
(12.8310,15.5172)
(12.4236,15.2500)
(12.2200,15.3846)
(12.0163,15.4856)
(11.8126,15.2632)
(11.6090,15.1194)
(11.4053,15.5125)
(11.2016,15.6250)
(10.9980,15.9292)
(10.7943,15.6805)
(10.5906,15.4303)
(10.3870,15.2695)
(10.1833,15.0602)
(9.9796,15.1703)
(9.7760,15.0000)
(9.5723,15.2104)
(9.3686,15.6997)
(9.1650,15.8451)
(8.9613,16.0584)
(8.7576,15.7509)
(8.5540,15.4412)
(8.3503,15.2416)
(8.1466,15.3846)
(7.9430,16.0494)
(7.7393,15.8996)
(7.5356,15.6780)
(7.3320,15.3191)
(7.1283,15.9817)
(6.9246,16.1137)
(6.7210,15.7895)
(6.5173,15.5340)
(6.3136,15.2709)
(6.1100,16.3043)
(5.9063,16.7630)
(5.7026,16.4706)
(5.2953,16.0494)
(5.0916,16.4474)
(4.8880,16.1074)
(4.6843,15.6463)
(4.4807,15.4930)
(4.2770,15.0000)
(4.0733,15.2672)
(3.8697,14.8438)
(3.6660,14.2857)
(3.4623,14.6552)
(3.2587,14.2857)
(3.0550,13.8889)
(2.8513,13.0841)
(2.6477,24.0741)
(2.4440,26.0870)
(2.2403,24.4444)
(2.0367,25.0000)
(1.8330,28.1250)
(1.6293,26.6667)
(1.4257,28.0000)
(1.2220,31.5789)
(1.0183,50.0000)
(0.8147,44.4444)
(0.6110,50.0000)
(0.2037,33.3333)
(0.0000,0.0000)
(0.0,0.0000)};

\addlegendentry{Our Full Method (AP = 39.85)}
\addlegendentry{Mix (AP = 11.14)}
\addlegendentry{Only Synthetic (AP = 9.67)}

==> figures/skew/argswap.tex <==
% cls ap
\addplot [draw=Peach, line width=0.7pt, densely dotted] coordinates {
  (1, 8.377850702)
  (2, 8.069457248)
  (4, 8.062462268)
  (8, 7.882986553)
  (16, 7.884887632)
  (32, 8.004236695)
  (64, 8.465051584)
  (176, 8.49)
};

% cls prec
\addplot [draw=Peach, line width=0.7pt,] coordinates {
  (1, 1.25)
  (2, 1.47)
  (4, 2.22)
  (8, 5.62)
  (16, 14.38)
  (32, 27.029999999999998)
  (64, 65.22)
  (176, 73.68)
};

% cls recall
\addplot [draw=Peach, line width=0.7pt, dashed] coordinates {
  (1, 50.0)
  (2, 29.270000000000003)
  (4, 21.54)
  (8, 14.23)
  (16, 8.94)
  (32, 8.129999999999999)
  (64, 6.1)
  (176, 5.6899999999999995)
};

% cls-loc prec
\addplot [draw=Plum, line width=0.7pt] coordinates {
  (1, 0.8999999999999999)
  (2, 1.25)
  (4, 1.97)
  (8, 5.140000000000001)
  (16, 14.38)
  (32, 27.029999999999998)
  (64, 65.22)
  (176, 73.68)
};

% cls-loc recall
\addplot [draw=Plum, line width=0.7pt, dashed] coordinates {
  (1, 36.18)
  (2, 24.8)
  (4, 19.11)
  (8, 13.01)
  (16, 8.94)
  (32, 8.129999999999999)
  (64, 6.1)
  (176, 5.6899999999999995)
};

% cls-loc-rep prec
\addplot [draw=Cerulean, line width=0.7pt] coordinates {
  (1, 0.7100000000000001)
  (2, 1.08)
  (4, 1.8399999999999999)
  (8, 5.140000000000001)
  (16, 14.38)
  (32, 27.029999999999998)
  (64, 65.22)
  (176, 73.68)
};

% cls-loc-rep recall
\addplot [draw=Cerulean, line width=0.7pt, dashed] coordinates {
  (1, 28.46)
  (2, 21.54)
  (4, 17.89)
  (8, 13.01)
  (16, 8.94)
  (32, 8.129999999999999)
  (64, 6.1)
  (176, 5.6899999999999995)
};

==> figures/skew/varmisuse.tex <==
% cls ap
\addplot [draw=Peach, line width=0.7pt, densely dotted] coordinates {
  (1, 7.40)
  (2, 8.75)
  (4, 9.72)
  (8, 11.97)
  (16, 14.49)
  (32, 16.41)
  (64, 18.95)
  (190, 20.96)
};

% cls prec
\addplot [draw=Peach, line width=0.7pt] coordinates {
  (1, 2.64)
  (2, 3.86)
  (4, 5.96)
  (8, 9.25)
  (16, 17.74)
  (32, 26.05)
  (64, 37.42)
  (190, 64.79)
};

% cls recall
\addplot [draw=Peach, line width=0.7pt, dashed] coordinates {
  (1, 71.13)
  (2, 53.27)
  (4, 36.31)
  (8, 27.08)
  (16, 22.92)
  (32, 18.45)
  (64, 17.26)
  (190, 13.69)
};

% cls-loc prec
\addplot [draw=Plum, line width=0.7pt] coordinates {
  (1, 1.45)
  (2, 2.50)
  (4, 4.39)
  (8, 7.52)
  (16, 15.67)
  (32, 23.53)
  (64, 35.48)
  (190, 61.97)
};

% cls-loc recall
\addplot [draw=Plum, line width=0.7pt, dashed] coordinates {
  (1, 38.99)
  (2, 34.52)
  (4, 26.79)
  (8, 22.02)
  (16, 20.24)
  (32, 16.67)
  (64, 16.37)
  (190, 13.10)
};

% cls-loc-rep prec
\addplot [draw=Cerulean, line width=0.7pt] coordinates {
  (1, 1.15)
  (2, 2.05)
  (4, 3.76)
  (8, 6.50)
  (16, 13.82)
  (32, 21.01)
  (64, 32.90)
  (190, 56.34)
};

% cls-loc-rep recall
\addplot [draw=Cerulean, line width=0.7pt, dashed] coordinates {
  (1, 30.95)
  (2, 28.27)
  (4, 22.92)
  (8, 19.05)
  (16, 17.86)
  (32, 14.88)
  (64, 15.18)
  (190, 11.90)
};

==> figures/skew/wrongbinop.tex <==
% cls ap
\addplot [draw=Peach, line width=0.7pt, densely dotted] coordinates {
  (1, 19.84)
  (2, 25.95)
  (4, 37.03)
  (8, 42.23)
  (16, 37.61)
  (32, 35.05)
  (64, 40.10)
  (100, 39.85)
};

% cls prec
\addplot [draw=Peach, line width=0.7pt] coordinates {
  (1, 7.35)
  (2, 10.79)
  (4, 19.00)
  (8, 27.56)
  (16, 34.40)
  (32, 38.94)
  (64, 47.47)
  (100, 52.30)
};

% cls recall
\addplot [draw=Peach, line width=0.7pt, dashed] coordinates {
  (1, 78.62)
  (2, 71.49)
  (4, 66.80)
  (8, 62.93)
  (16, 61.51)
  (32, 57.03)
  (64, 47.86)
  (100, 43.99)
};

% cls-loc prec
\addplot [draw=Plum, line width=0.7pt] coordinates {
  (1, 6.65)
  (2, 10.18)
  (4, 18.08)
  (8, 26.67)
  (16, 33.26)
  (32, 37.97)
  (64, 46.46)
  (100, 51.09)
};

% cls-loc recall
\addplot [draw=Plum, line width=0.7pt, dashed] coordinates {
  (1, 71.08)
  (2, 67.41)
  (4, 63.54)
  (8, 60.90)
  (16, 59.47)
  (32, 55.60)
  (64, 46.84)
  (100, 42.97)
};

% cls-loc-rep prec
\addplot [draw=Cerulean, line width=0.7pt] coordinates {
  (1, 5.94)
  (2, 9.38)
  (4, 16.86)
  (8, 25.51)
  (16, 32.00)
  (32, 37.00)
  (64, 45.05)
  (100, 49.64)
};

% cls-loc-rep recall
\addplot [draw=Cerulean, line width=0.7pt, dashed] coordinates {
  (1, 63.54)
  (2, 62.12)
  (4, 59.27)
  (8, 58.25)
  (16, 57.23)
  (32, 54.18)
  (64, 45.42)
  (100, 41.75)
};

==> figures/synthetic/argswap.tex <==
% cls ap
\addplot [draw=Peach, line width=0.7pt, densely dotted] coordinates {
  (0, 5.028230714999999)
  (1, 4.113446694)
  (2, 11.544474220000001)
  (4, 8.891902826)
  (8, 10.238865599999999)
  (16, 11.0439941)
  (32, 11.71090317)
  (64, 9.614711585999999)  
  (100, 8.49)
};

% cls prec
\addplot [draw=Peach, line width=0.7pt] coordinates {
  (0, 0.0)
  (1, 0.0)
  (2, 78.57)
  (4, 83.33)
  (8, 70.0)
  (16, 76.19)
  (32, 94.12)
  (64, 82.35)
  (100, 73.68)  
};

% cls recall
\addplot [draw=Peach, line width=0.7pt, dashed] coordinates {
  (0, 0.0)
  (1, 0.0)
  (2, 4.47)
  (4, 4.07)
  (8, 5.6899999999999995)
  (16, 6.5)
  (32, 6.5)
  (64, 5.6899999999999995)
  (100, 5.6899999999999995)
};

% cls-loc prec
\addplot [draw=Plum, line width=0.7pt] coordinates {
  (0, 0.0)
  (1, 0.0)
  (2, 78.57)
  (4, 83.33)
  (8, 70.0)
  (16, 76.19)
  (32, 94.12)
  (64, 82.35)
  (100, 73.68)  
};

% cls-loc recall
\addplot [draw=Plum, line width=0.7pt, dashed] coordinates {
  (0, 0.0)
  (1, 0.0)
  (2, 4.47)
  (4, 4.07)
  (8, 5.6899999999999995)
  (16, 6.5)
  (32, 6.5)
  (64, 5.6899999999999995)
  (100, 5.6899999999999995)  
};

% cls-loc-rep prec
\addplot [draw=Cerulean, line width=0.7pt] coordinates {
  (0, 0.0)
  (1, 0.0)
  (2, 71.43)
  (4, 75.0)
  (8, 60.0)
  (16, 76.19)
  (32, 88.24)
  (64, 82.35)
  (100, 73.68)
};

% cls-loc-rep recall
\addplot [draw=Cerulean, line width=0.7pt, dashed] coordinates {
  (0, 0.0)
  (1, 0.0)
  (2, 4.07)
  (4, 3.66)
  (8, 4.88)
  (16, 6.5)
  (32, 6.1)
  (64, 5.6899999999999995)
  (100, 5.6899999999999995)  
};

==> figures/synthetic/varmisuse.tex <==
% cls ap
\addplot [draw=Peach, line width=0.7pt, densely dotted] coordinates {
  (0, 4.601139038)
  (1, 3.940259356)
  (2, 4.815292782)
  (4, 3.505218526)
  (8, 6.083424685)
  (16, 12.27075108)
  (32, 15.43976349)
  (64, 18.24246477)
  (100, 20.96)
};

% cls prec
\addplot [draw=Peach, line width=0.7pt] coordinates {
  (0.8, 0)
  (2, 0)
  (4, 0)
  (8, 0)
  (16, 76.19)
  (32, 62.50)
  (64, 54.24)
  (100, 64.79)
};

% cls recall
\addplot [draw=Peach, line width=0.7pt, dashed] coordinates {
  (0.8, 0)
  (2, 0)
  (4, 0)
  (8, 0)
  (16, 4.76)
  (32, 7.44)
  (64, 9.52)
  (100, 13.69)
};

% cls-loc prec
\addplot [draw=Plum, line width=0.7pt] coordinates {
  (0.8, 0)
  (2, 0)
  (4, 0)
  (8, 0)
  (16, 76.19)
  (32, 62.50)
  (64, 50.85)
  (100, 61.97)
};

% cls-loc recall
\addplot [draw=Plum, line width=0.7pt, dashed] coordinates {
  (0.8, 0)
  (2, 0)
  (4, 0)
  (8, 0)
  (16, 4.76)
  (32, 7.44)
  (64, 8.93)
  (100, 13.10)
};

% cls-loc-rep prec
\addplot [draw=Cerulean, line width=0.7pt] coordinates {
  (0.8, 0)
  (2, 0)
  (4, 0)
  (8, 0)
  (16, 71.43)
  (32, 62.50)
  (64, 49.15)
  (100, 56.34)
};

% cls-loc-rep recall
\addplot [draw=Cerulean, line width=0.7pt, dashed] coordinates {
  (0.8, 0)
  (2, 0)
  (4, 0)
  (8, 0)
  (16, 4.46)
  (32, 7.44)
  (64, 8.63)
  (100, 11.90)
};

==> figures/synthetic/wrongbinop.tex <==
% cls ap
\addplot [draw=Peach, line width=0.7pt, densely dotted] coordinates {
  (0, 29.9902825)
  (1, 21.89839995)
  (2, 32.27391063)
  (4, 35.3610703)
  (8, 39.1555756)
  (16, 33.620907)
  (32, 37.84622526)
  (64, 39.30929389)
  (100, 39.85)
};

% cls prec
\addplot [draw=Peach, line width=0.7pt] coordinates {
  (0.8, 47.74)
  (2, 54.03)
  (4, 51.82)
  (8, 53.55)
  (16, 49.07)
  (32, 46.95)
  (64, 49.32)
  (100, 52.30)
};

% cls recall
\addplot [draw=Peach, line width=0.7pt, dashed] coordinates {
  (0.8, 25.87)
  (2, 36.86)
  (4, 40.53)
  (8, 39.92)
  (16, 42.97)
  (32, 40.73)
  (64, 44.40)
  (100, 43.99)
};

% cls-loc prec
\addplot [draw=Plum, line width=0.7pt] coordinates {
  (0.8, 45.49)
  (2, 51.94)
  (4, 50.26)
  (8, 52.46)
  (16, 47.91)
  (32, 46.24)
  (64, 48.42)
  (100, 51.09)
};

% cls-loc recall
\addplot [draw=Plum, line width=0.7pt, dashed] coordinates {
  (0.8, 24.64)
  (2, 35.44)
  (4, 39.31)
  (8, 39.10)
  (16, 41.96)
  (32, 40.12)
  (64, 43.58)
  (100, 42.97)
};

% cls-loc-rep prec
\addplot [draw=Cerulean, line width=0.7pt] coordinates {
  (0.8, 42.11)
  (2, 47.76)
  (4, 45.83)
  (8, 49.73)
  (16, 46.05)
  (32, 45.31)
  (64, 47.51)
  (100, 49.64)
};

% cls-loc-rep recall
\addplot [draw=Cerulean, line width=0.7pt, dashed] coordinates {
  (0.8, 22.81)
  (2, 32.59)
  (4, 35.85)
  (8, 37.07)
  (16, 40.33)
  (32, 39.31)
  (64, 42.77)
  (100, 41.75)
};

==> tables/numbugs.tex <==
\begin{wraptable}{r}{0.20\textwidth}
  \vspace{-3mm}
  \scriptsize
  \centering
  \def\arraystretch{1.1}
  \setlength\tabcolsep{4pt}
  \begin{tabular}{@{}lrr@{}}
    \toprule
    Bug Type & Ours & \pypibugs{} \\
    \midrule
    \texttt{\tiny var-misuse} & \textbf{1309} & 1278 \\
    \texttt{\tiny wrong-binop} & \textbf{1719} & 680 \\
    \texttt{\tiny arg-swap} & \textbf{932} & 283 \\
    All & \textbf{3960} & 2374 \\
    \bottomrule
  \end{tabular}
  \vspace{-2mm}
\end{wraptable}
